Characterizing the Expressivity of Local Attention in Transformers

The transformer is the most popular neural architecture for language modeling. The cornerstone of the transformer is its global attention mechanism, which lets the model aggregate information from all preceding tokens before generating the next token. One common variant of attention is called local attention, which restricts each token to aggregating information from a bounded window of predecessors, reducing the quadratic cost of global attention to linear. Although this restriction is usually motivated by efficiency, it has also been found to improve model quality, a phenomenon that has so far lacked a satisfactory explanation. We provide a formal account of this phenomenon in terms of recognizer expressivity. It has been shown that fixed-precision transformers with global attention correspond to a fragment of linear temporal logic containing a single past operator. We additionally prove that adding local attention introduces a second temporal operator, strictly enlarging the class of recognizable regular languages. Moreover, global and local attention are expressively complementary: neither subsumes the other, and combining them yields the richest fragment. Experiments on formal language recognition and natural language modeling corroborate the theory, showing that hybrid global--local transformers outperform their global-only counterparts.

==> macros.tex <==
\newcommand{\mymacro}[1]{{#1}}
\newcommand{\algmacro}[1]{{\color{ETHBronze} #1}}
\newcommand{\hiddmacro}[1]{{\color{ETHGreen} #1}}

\usepackage{ellipsis}
\makeatletter
\renewcommand*{\mathellipsis}{%
  \mathinner{%
    \kern\ellipsisbeforegap%
    {\ldotp}\kern\ellipsisgap%
    {\ldotp}\kern\ellipsisgap%
    {\ldotp}\kern\ellipsisaftergap%
  }%
}
\renewcommand*{\dotsb@}{%
  \mathinner{%
    \kern\ellipsisbeforegap%
    {\cdotp}\kern\ellipsisgap%
    {\cdotp}\kern\ellipsisgap%
    {\cdotp}\kern\ellipsisaftergap%
  }%
}
\renewcommand*{\@cdots}{%
  \mathinner{%
    \kern\ellipsisbeforegap%
    {\cdotp}\kern\ellipsisgap%
    {\cdotp}\kern\ellipsisgap%
    {\cdotp}\kern\ellipsisaftergap%
  }%
}
\renewcommand*{\ellipsis@default}{%
  \ellipsis@before
  \kern\ellipsisbeforegap
  .\kern\ellipsisgap
  .\kern\ellipsisgap
  .\kern\ellipsisgap
  \ellipsis@after\relax}
\renewcommand*{\ellipsis@centered}{%
  \ellipsis@before
  \kern\ellipsisbeforegap
  .\kern\ellipsisgap
  .\kern\ellipsisgap
  .\kern\ellipsisaftergap
  \ellipsis@after\relax}
\AtBeginDocument{%
  \DeclareRobustCommand*{\dots}{%
    \ifmmode\@xp\mdots@\else\@xp\textellipsis\fi}}
\def\ellipsisgap{-.05em}
\def\ellipsisbeforegap{-.05em}
\def\ellipsisaftergap{.05em}
\makeatother


\newcommand{\mathhl}[2][yellow!80]{\mathchoice%
    {\colorbox{#1}{$\displaystyle#2$}}%
    {\colorbox{#1}{$\textstyle#2$}}%
    {\colorbox{#1}{$\scriptstyle#2$}}%
    {\colorbox{#1}{$\scriptscriptstyle#2$}}}%

\newcommand{\timestamp}{\ddmmyyyydate\today \,\,- \currenttime h}

\newcommand{\defn}[1]{\textbf{#1}}

\newcommand{\paroutline}[3][false]{%
    \ifnum\pdfstrcmp{#1}{true}=0
        #3%
    \else
        [\textit{\textcolor{DiverseMagenta}{#2}}] \textcolor{AccentBlue}{#3}%
    \fi
}

\newcommand{\anejchange}[1]{\textcolor{ETHRed}{#1}}
\newcommand{\claudetext}[1]{\textcolor{red}{#1}}
\newcommand{\operators}{\opcolor{\mathcal{O}}}
\definecolor{OperatorColor}{RGB}{0,110,65}    %
\definecolor{FormulaColor}{RGB}{175,70,30}    %
\definecolor{StringColor}{RGB}{20,55,135}     %
\definecolor{LTLColor}{RGB}{110,30,55}        %
\newcommand{\opcolor}[1]{{\color{OperatorColor} #1}}
\newcommand{\fmcolor}[1]{{\color{FormulaColor} #1}}
\newcommand{\strcolor}[1]{{\color{StringColor} #1}}
\newcommand{\ltlcolor}[1]{{\color{LTLColor} #1}}

\newcommand{\vbeta}{{\mymacro{\boldsymbol{\beta}}}}
\newcommand{\valpha}{{\mymacro{\boldsymbol{\alpha}}}}
\newcommand{\vlambda}{{\mymacro{\boldsymbol{\lambda}}}}
\newcommand{\veta}{{\mymacro{\boldsymbol{\eta}}}}
\newcommand{\vgamma}{{\mymacro{\boldsymbol{\gamma}}}}
\newcommand{\ptheta}{{\mymacro{p_{\vtheta}}}}
\newcommand{\inv}[1]{{\mymacro{#1^{-1}}}}
\newcommand{\hidd}[1]{{\mymacro{y_{#1}}}}
\newcommand{\obs}[1]{{\mymacro{x_{#1}}}}
\newcommand{\hidds}{{\mymacro{\mathbf{Y}}}}
\newcommand{\obss}{{\mymacro{\mathbf{X}}}}
\newcommand{\hiddspace}{{\mymacro{\mathcal{Y}}}}
\newcommand{\obsspace}{{\mymacro{ \mathcal{X}}}}
\newcommand{\transm}{{\mymacro{\bT}}}
\newcommand{\emissm}{{\mymacro{\bE}}}
\newcommand{\weights}{{\mymacro{\bw}}}
\newcommand{\biasScalar}{{\mymacro{ b}}}
\newcommand{\biasVector}{{\mymacro{ \vb}}}
\newcommand{\featuref}{{\mymacro{ \mathbf{f}}}}

\newcommand{\pathval}{{\mymacro{\mathrm{R}}}}
\newcommand{\valueset}{{\mymacro{\mathrm{V}}}}
\newcommand{\expectation}{{\mymacro{\mathbb{E}}}}
\newcommand{\pdens}{{\mymacro{ p}}}
\newcommand{\pdensBar}{{\mymacro{ \bar{\pdens}}}}
\newcommand{\pdensTildeEOS}{{\mymacro{ \tilde{\pdens}_\eos}}}
\newcommand{\qdens}{{\mymacro{ q}}}
\newcommand{\loglikelihood}{{\mymacro{ \ell\ell}}}
\newcommand{\samplespace}{{\mymacro{ \Omega}}}
\newcommand{\eventspace}{{\mymacro{ \mathcal{F}}}}
\newcommand{\eventspaceA}{{\mymacro{ \mathcal{A}}}}
\newcommand{\probmeasure}{{\mymacro{ \mathbb{P}}}}
\newcommand{\probfunction}{{\mymacro{ \mathbb{P}}}}
\newcommand{\pushfwdMeasure}{{\mymacro{ \probfunction_*}}}
\newcommand{\probtuple}{{\mymacro{\left(\samplespace, \eventspace, \probfunction\right)}}}
\newcommand{\bomega}{{\mymacro{ \bm{\omega}}}}
\newcommand{\overC}{{\mymacro{ \overline{C}}}}
\newcommand{\overcalC}{{\mymacro{ \overline{\mathcal{C}}}}}
\newcommand{\calC}{{\mymacro{ \mathcal{C}}}}
\newcommand{\strCount}{{\mymacro{ C}}}


\newcommand{\paramspace}{{\mymacro{\boldsymbol{\Theta}}}}
\newcommand{\param}{{\mymacro{\theta}}}
\newcommand{\modelparam}{{\mymacro{\theta}}}
\newcommand{\params}{{\mymacro{\vtheta}}}
\newcommand{\modelparams}{{\mymacro{\vtheta}}}
\newcommand{\modelparamstrue}{{\mymacro{\modelparams^\star}}}
\newcommand{\modelparamsopt}{{\mymacro{\widehat\modelparams}}}
\newcommand{\premodel}{{\mymacro{g_{\scaleto{\modelparams}{4pt}}}}} %
\newcommand{\model}{{\mymacro{p_{\scaleto{\modelparams}{4pt}}}}}
\newcommand{\modelopt}{{\mymacro{p_{\scaleto{\modelparamsopt}{4pt}}}}}

\newcommand{\ind}[1]{\mathbbm{1} \left\{ #1 \right\}}

\newcommand{\floor}[1]{\mymacro{\left\lfloor #1 \right\rfloor}}
\newcommand{\fieldd}{{\mymacro{ \mathbb{F}^d}}}
\newcommand{\field}{{\mymacro{ \mathbb{F}}}}
\newcommand{\vectorspace}{{\mymacro{ \mathbb{V}}}}
\newcommand{\vspacedim}{{\mymacro{ D}}}
\newcommand{\Q}{{\mymacro{ \mathbb{Q}}}}
\newcommand{\R}{{\mymacro{ \mathbb{R}}}}
\newcommand{\Rex}{{\mymacro{ \overline{\R}}}}
\newcommand{\Rd}{{\mymacro{ \R^d}}}
\newcommand{\RD}{{\mymacro{ \R^D}}}
\newcommand{\RDD}{{\mymacro{ \R^{D \times D}}}}
\newcommand{\C}{{\mymacro{ \mathbb{C}}}}
\newcommand{\Z}{{\mymacro{ \mathbb{Z}}}}
\newcommand{\B}{{\mymacro{ \mathbb{B}}}}
\newcommand{\BD}{{\mymacro{ \B^D}}}
\newcommand{\BDD}{{\mymacro{ \B^{D \times D}}}}
\newcommand{\Bset}{{\mymacro{ \set{0, 1}}}}
\newcommand{\Rplus}{{\mymacro{ \mathbb{R}_{+}}}}
\newcommand{\Rnonnegative}{{\mymacro{ \mathbb{R}_{\geq 0}}}}
\newcommand{\Rminus}{{\mymacro{ \mathbb{R}_{-}}}}
\newcommand{\sigalgebra}{{\mymacro{ \sigma\text{-}\text{algebra}}}}
\newcommand{\func}{{\mymacro{ f}}}
\newcommand{\funcg}{{\mymacro{ g}}}
\newcommand{\vfunc}{{\mymacro{ \mathbf{f}}}}
\newcommand{\hatvfunc}{{\mymacro{ \hat{\mathbf{f}}}}}
\newcommand{\vfuncg}{{\mymacro{ \mathbf{g}}}}
\newcommand{\diag}[1]{{\mymacro{ \mathrm{diag}\!\left(#1\right)}}}
\newcommand{\norm}[1]{{\mymacro{ \left\lVert #1 \right\rVert}}}
\newcommand{\abs}[1]{{\mymacro{ \left| #1 \right|}}}
\newcommand{\normsubone}[1]{\mymacro{ \left\lVert #1 \right\rVert_{1}}}
\newcommand{\normsubtwo}[1]{\mymacro{ \left\lVert #1 \right\rVert_{2}}}
\newcommand{\normsubinf}[1]{\mymacro{ \left\lVert #1 \right\rVert_{\infty}}}
\newcommand{\relation}{{\mymacro{ R}}}
\newcommand{\equivClass}[1]{{\mymacro{ \left[#1\right]}}}
\newcommand{\eval}{{\mymacro{ \lambda}}}
\newcommand{\evecv}{{\mymacro{ \vv}}}
\newcommand{\evecu}{{\mymacro{ \vu}}}
\newcommand{\lambdamax}{{\mymacro{\lambda_{\text{max}}}}}
\newcommand{\evalmax}{{\mymacro{\eval_{\text{max}}}}}
\newcommand{\ordering}{{\mymacro{ n}}}
\newcommand{\inner}[2]{{\mymacro{ #1^\top #2}}}
\newcommand{\innerProd}[2]{{\mymacro{ \left\langle #1, #2 \right\rangle }}}
\newcommand{\basisVect}{{\mymacro{ \ve}}}
\newcommand{\perm}{{\mymacro{ \pi}}}
\newcommand{\permFun}[1]{{\perm\left(#1\right)}}
\newcommand{\lipschitzConstant}{{\mymacro{\lambda}}}
\newcommand{\lipschitzFun}[1]{{\lipschitzConstant_{#1}}}
\newcommand{\lipschitzPrimeFun}[1]{{\lipschitzConstant_{#1}'}}
\newcommand{\funcBoundConstant}{{\mymacro{C}}}
\newcommand{\boundFun}[1]{{\funcBoundConstant_{#1}}}

\newcommand{\alphabet}{{\strcolor{ \Sigma}}}
\newcommand{\alphabetchar}{{\mymacro{ \Sigma_0}}}
\newcommand{\alphabettree}{{\mymacro{ \mathcal{T}}}}
\newcommand{\alphabetmerge}{\mymacro{ \Upsilon_{\alphabet}}}
\newcommand{\stackalphabet}{{\mymacro{ \Gamma}}}
\newcommand{\oalphabet}{{\mymacro{ \Delta}}}
\newcommand{\outalphabet}{\oalphabet}
\newcommand{\eosalphabet}{{\mymacro{ \overline{\alphabet}}}}
\newcommand{\bosalphabet}{{\mymacro{ \underline{\alphabet}}}}
\newcommand{\kleene}[1]{{\mymacro{#1^*}}}
\newcommand{\kleeneplus}[1]{{\mymacro{#1^+}}}
\newcommand{\rankedalphabet}{{\mymacro{ \left(\alphabet, \arity)\right}}}
\newcommand{\regex}{{\mymacro{ \alpha}}}

\newcommand{\str}{{\strcolor{\textbf{\texttt{w}}}}}
\newcommand{\strlt}{{\mymacro{ \str_{<\tstep}}}}
\newcommand{\strlet}{{\mymacro{ \str_{\leq\tstep}}}}
\newcommand{\strltplus}{{\mymacro{ \str_{<\tstep+1}}}}
\newcommand{\strgt}{{\mymacro{ \str_{>\tstep}}}}
\newcommand{\strPrime}{{\mymacro{ \str'}}}
\newcommand{\eosstr}{{\mymacro{\overline{\str}}}}
\newcommand{\strlen}{{\mymacro{T}}}
\newcommand{\strs}{{\strcolor{\textbf{\texttt{s}}}}}
\newcommand{\strt}{{\strcolor{\textbf{\texttt{t}}}}}
\newcommand{\strx}{{\strcolor{\textbf{\texttt{x}}}}}
\newcommand{\stry}{{\strcolor{\textbf{\texttt{y}}}}}
\newcommand{\strz}{{\strcolor{\textbf{\texttt{z}}}}}
\newcommand{\stru}{{\strcolor{\textbf{\texttt{u}}}}}
\newcommand{\strv}{{\strcolor{\textbf{\texttt{v}}}}}
\newcommand{\eossym}{{\mymacro{\sym}}}
\newcommand{\symx}{{\mymacro{x}}}
\newcommand{\symz}{{\mymacro{z}}}
\newcommand{\stacksym}{{\mymacro{\stacksymbol{\gamma}}}}

\newcommand{\defeq}{\mathrel{\stackrel{\textnormal{\tiny def}}{=}}}

\newcommand{\NTo}[1]{{\mymacro{\left[ #1 \right]}}}
\newcommand{\Zmod}[1]{{\mymacro{\Z_{#1}}}}
\newcommand{\set}[1]{{\mymacro{\left\{ #1 \right\}}}}
\newcommand{\powerset}[1]{{\mymacro{\mathcal{P}{\left(#1\right)}}}}
\newcommand{\setcomplement}[1]{{\mymacro{#1^{\textsf{c}}}}}
\newcommand{\binv}[1]{{\mymacro{\left(#1\right)^{-1}}}}

\newcommand{\TODO}{{\color{red} TODO }}
\newcommand{\draft}[1]{{\color{AccentOrange} #1 }}

\newcommand{\justification}[1]{\tag*{\footnotesize{\textcolor{black!50}{#1}}}}

\newcommand{\textexample}[1]{{\mymacro{ \fontfamily{ppl}\selectfont \text{``#1''}}}}

\newcommand{\bigo}{{\mymacro{ \mathcal{O}}}}
\newcommand{\idx}{{\mymacro{ n}}}
\newcommand{\idxn}{{\mymacro{ n}}}
\newcommand{\idxd}{{\mymacro{ d}}}
\newcommand{\idxi}{{\mymacro{ i}}}
\newcommand{\idxj}{{\mymacro{ j}}}
\newcommand{\idxk}{{\mymacro{ k}}}
\newcommand{\idxl}{{\mymacro{ l}}}
\newcommand{\idxm}{{\mymacro{ m}}}
\newcommand{\setsize}{{\mymacro{ N}}}
\newcommand{\nsamples}{{\mymacro{ N}}}
\newcommand{\seqlength}{{\mymacro{ L}}}
\newcommand{\othseqlength}{{\mymacro{ M}}}
\newcommand{\nstates}{{\mymacro{ |\states|}}}
\newcommand{\nsymbols}{{\mymacro{ |\alphabet|}}}
\newcommand{\eosnsymbols}{{\mymacro{ |\eosalphabet|}}}
\newcommand{\bosnsymbols}{{\mymacro{ |\bosalphabet|}}}
\newcommand{\nsymbolsplus}{{\mymacro{\nsymbols + 1}}}
\newcommand{\tstep}{{\mymacro{ t}}}
\newcommand{\tstepminus}{{\mymacro{\tstep - 1}}}
\newcommand{\finaltstep}{{\mymacro{ T}}}

\newcommand{\pM}{\mymacro{\pdens}}
\newcommand{\pLM}{\mymacro{\pdens}}
\newcommand{\qLM}{\mymacro{\qdens}}
\newcommand{\pLNSM}{\mymacro{\pdens}}
\newcommand{\pLNSMFun}[2]{{\mymacro{\pLNSM\left(#1\mid#2\right)}}}
\newcommand{\pPrefix}{{\mymacro{ \pi}}}
\newcommand{\pGN}{\mymacro{\pdens}}
\newcommand{\pLN}{\mymacro{\pdens}}
\newcommand{\pLNbar}{{\mymacro{ \overline{p}_{\scaleto{\text{LN}}{4pt}}}}}
\newcommand{\scoringfunc}{{\mymacro{ \widehat{p}}}}
\newcommand{\unnormalizedpGN}{{\mymacro{ \scoringfunc_{\scaleto{\text{GN}}{4pt}}}}}
\newcommand{\unnormalizedpLN}{{\mymacro{ \scoringfunc_{\scaleto{\text{LN}}{4pt}}}}}
\newcommand{\unnormalizedpM}{{\mymacro{ \scoringfunc_{\scaleto{\text{M}}{4pt}}}}}
\newcommand{\unnormalizedpLM}{{\mymacro{ \scoringfunc_{\scaleto{\text{LM}}{4pt}}}}}
\newcommand{\pSM}{{\mymacro{ p_{\scaleto{\text{SM}}{4pt}}}}}
\newcommand{\pMLM}{{\mymacro{ p_{\scaleto{\texttt{MLM}}{4pt}}}}}
\newcommand{\pASM}{{\mymacro{ p_{\scaleto{\text{ASM}}{4pt}}}}}
\newcommand{\bos}{{\mymacro{\textsc{bos}}}}
\newcommand{\eos}{{\mymacro{\textsc{eos}}}}
\newcommand{\unk}{{\mymacro{\textsc{unk}}}}
\newcommand{\ngr}{{\mymacro{ \textit{n}}}}
\newcommand{\ngram}{{\mymacro{ \textit{n}-gram}}\xspace}
\newcommand{\nStrictLocal}{{\mymacro{ \text{SL}_\ngr}}}
\newcommand{\strictLocal}{{\mymacro{ \text{SL}}}}
\newcommand{\kslAcr}{{\mymacro{\text{SL}_{\locPar}}}}
\newcommand{\slAcr}{{\mymacro{\text{SL}}}\xspace}
\newcommand{\normConstant}{{\mymacro{ Z}}}
\newcommand{\featurespacedim}{{\mymacro{ d}}}
\newcommand{\embedDim}{{\mymacro{ R}}}
\newcommand{\scoref}{{\mymacro{ \func}}}
\newcommand{\similarity}{{\mymacro{ \texttt{sim}}}}
\newcommand{\ctxLogits}[1]{{\mymacro{ \vw\left(#1\right)}}}

\newcommand{\dyck}[1]{{\mymacro{ \mathrm{D}\!\left(#1\right)}}}
\newcommand{\boundedDyck}[2]{{\mymacro{ \mathrm{D}\!\left(#1, #2\right)}}}
\newcommand{\nBracketTypes}{{\mymacro{ k}}}
\newcommand{\dyckMaxDepth}{{\mymacro{ m}}}
\newcommand{\openBr}[1]{{\mymacro{ \langle_{#1}}}}
\newcommand{\closeBr}[1]{{\mymacro{ \rangle_{#1}}}}
\newcommand{\binEnc}[1]{{\mymacro{ \texttt{bin}\!\left(#1\right)}}}
\newcommand{\hToQ}{{\mymacro{ s}}}
\newcommand{\hToQFun}[1]{{\mymacro{ \hToQ \!\left( #1 \right)}}}
\newcommand{\hToQinv}{{\mymacro{ \inv{s}}}}
\newcommand{\hToQinvFun}[1]{{\mymacro{ \hToQinv\!\left( #1 \right)}}}
\newcommand{\qToH}{{\mymacro{ h}}}
\newcommand{\qToHFun}[1]{{\mymacro{ \qToH \!\left( #1 \right)}}}
\newcommand{\qToHinv}{{\mymacro{ \inv{h}}}}
\newcommand{\qToHinvFun}[1]{{\mymacro{ \qToHinv\!\left( #1 \right)}}}
\newcommand{\strToQ}[1]{{\mymacro{\!\left[ #1 \right]}}}
\newcommand{\sinkState}{{\mymacro{ \textsf{R}}}}
\newcommand{\acceptState}{{\mymacro{ \textsf{A}}}}

\newcommand{\inEmbedding}{{\mymacro{ \vr}}}
\newcommand{\inEmbeddingFun}[2][]{{\mymacro{ \inEmbedding\!\left(#2\right)}}}
\newcommand{\embedSym}{{\mymacro{ \embedding{\sym}}}}
\newcommand{\inEmbedSym}{{\mymacro{ \inEmbeddingFun{\sym}}}}
\newcommand{\inEmbedSymt}{{\mymacro{ \inEmbeddingFun{\sym_\tstep}}}}
\newcommand{\inEmbedSymtminus}{{\mymacro{ \inEmbeddingFun{\sym_{\tstep - 1}}}}}
\newcommand{\embedMtx}{{\mymacro{ \mE}}}
\newcommand{\eembedMtx}{{\mymacro{ \emE}}}
\newcommand{\embedEOS}{{\mymacro{ \embedding{\eos}}}}
\newcommand{\embedStr}{{\mymacro{ \embedding{\str}}}}
\newcommand{\embedSymt}{{\mymacro{ \embedding{{\sym_\tstep}}}}}
\newcommand{\embedSymtminus}{{\mymacro{ \embedding{{\sym_{\tstep-1}}}}}}
\newcommand{\embedSymPrime}{{\mymacro{ \embedding{{\sym'}}}}}

\newcommand{\symlt}{{\mymacro{ \sym_{<\tstep}}}}
\newcommand{\symt}{{\mymacro{ \sym_{\tstep}}}}
\newcommand{\symT}{{\mymacro{ \sym_{\strlen}}}}
\newcommand{\symi}{{\mymacro{ \sym_{i}}}}
\newcommand{\symtminus}{{\mymacro{ \sym_{\tstep-1}}}}
\newcommand{\symtplus}{{\mymacro{ \sym_{\tstep+1}}}}
\newcommand{\symzero}{{\mymacro{ \sym_{0}}}}
\newcommand{\symone}{{\mymacro{ \sym_{1}}}}
\newcommand{\symTminus}{{\mymacro{ \sym_{T-1}}}}
\newcommand{\symPrime}{{\mymacro{ \sym'}}}

\newcommand{\bias}{{\mymacro{ \vb}}}
\newcommand{\biasSym}{{\mymacro{ b_\sym}}}
\newcommand{\biasSymt}{{\mymacro{ b_{\sym_\tstep}}}}
\newcommand{\biasSymtminus}{{\mymacro{ b_{\sym_{\tstep-1}}}}}
\newcommand{\biasSymPrime}{{\mymacro{ b_{\symPrime}}}}
\newcommand{\biasStr}{{\mymacro{ b_\str}}}
\newcommand{\biasStrPrime}{{\mymacro{ b_{\strPrime}}}}
\newcommand{\biasVech}{{\mymacro{ \vb}}}
\newcommand{\biasVecy}{{\mymacro{ \vb_{y}}}}
\newcommand{\biasVeco}{{\mymacro{ \vb_{o}}}}

\newcommand{\vot}{{\mymacro{ \vo_{t}}}}
\newcommand{\votminus}{{\mymacro{ \vo_{t-1}}}}

\newcommand{\autoregmodel}{{\mymacro{ autoregressive sequence model\xspace}}}
\newcommand{\autoregmodelAcronym}{{\mymacro{ ASM\xspace}}}
\newcommand{\GNMAcronym}{{\mymacro{ GNM\xspace}}}
\newcommand{\LNMAcronym}{{\mymacro{ LNM\xspace}}}
\newcommand{\SMAcronym}{{\mymacro{ SM\xspace}}}

\newcommand{\queue}{{\mymacro{\textsf{queue}}}}
\newcommand{\stack}{{\mymacro{\textsf{stack}}}}
\newcommand{\inblock}{{\mymacro{\textsf{in-block}}}}

\newcommand{\graph}{\mymacro{ \mathcal{G}}}
\newcommand{\scc}{\mymacro{ \mathcal{S}}}

\newcommand{\semiring}{{\mymacro{ \mathcal{W}}}}
\newcommand{\semiringtuple}{{\mymacro{\left(\semiringset, \oplus, \otimes, \zero, \one \right)}}}
\newcommand{\closedsemiringtuple}{{\mymacro{ \left(\semiringset, \oplus, \otimes, \zero, \one, \kleene{} \right)}}}
\newcommand{\semiringset}{{\mymacro{ \mathbb{K}}}}
\newcommand{\zero}{{\mymacro{\mathbf{0}}}}
\newcommand{\one}{{\mymacro{\mathbf{1}}}}
\newcommand{\matrixsemiringset}{{\mymacro{ \mathbf{M}_{D}\left( \semiring \right) }}}
\newcommand{\booleansemiring}{{\mymacro{\left(\set{0, 1}, \vee, \wedge, \textsc{true}, \textsc{false} \right)}}}
\newcommand{\tropicalsemiring}{{\mymacro{\left(\Rplus, \min, +, \infty, 0 \right)}}}
\newcommand{\probabilitysemiring}{{\mymacro{\left(\left[0, 1\right], +, \times, 0, 1 \right)}}}
\newcommand{\realssemiring}{{\mymacro{\left(\R, +, \times, 0, 1 \right)}}}
\newcommand{\positiverealssemiring}{{\mymacro{\left(\Rplus, +, \times, 0, 1 \right)}}}
\newcommand{\nonnegativerealssemiring}{{\mymacro{\left(\Rnonnegative, +, \times, 0, 1 \right)}}}

\newcommand{\automaton}{{\algmacro{ \mathcal{A}}}}
\newcommand{\wfsa}{{\mymacro{ \automaton}}}
\newcommand{\transducer}{{\mymacro{ \mathcal{T}}}}
\newcommand{\wfst}{{\mymacro{ \transducer}}}
\newcommand{\detautomaton}{{\mymacro{ \automaton_{\textsc{det}}}}}
\newcommand{\pushedautomaton}{{\mymacro{ \automaton_{\textsc{push}}}}}
\newcommand{\minautomaton}{{\mymacro{ \automaton_{\textsc{min}}}}}
\newcommand{\epsautomaton}{{\mymacro{ \automaton_{\neg\varepsilon}}}}
\newcommand{\trimautomaton}{{\mymacro{ \automaton_{\textsc{trim}}}}}
\newcommand{\unionautomaton}{{\mymacro{ \automaton_{\textsc{union}}}}}
\newcommand{\complementautomaton}{{\mymacro{ \automaton_{\textsc{c}}}}}
\newcommand{\intersectautomaton}{{\mymacro{ \automaton_{\textsc{intersect}}}}}
\newcommand{\epsonlyautomaton}{{\mymacro{ \automaton_{\varepsilon}}}}
\newcommand{\closure}{{\mymacro{ \kappa}}}
\newcommand{\stateq}{{\mymacro{ q}}}
\newcommand{\statep}{{\mymacro{ p}}}
\newcommand{\stater}{{\mymacro{ r}}}
\newcommand{\states}{{\mymacro{ Q}}}
\newcommand{\stackstates}{{\mymacro{ Z}}}
\newcommand{\trans}{{\mymacro{ \delta}}}
\newcommand{\projectstates}{{\mymacro{ \mathcal{E}_{\states}}}}
\newcommand{\outarcs}{{\mymacro{ \mathcal{E}}}}
\newcommand{\inarcs}{{\mymacro{ \inv{\mathcal{E}}}}}
\newcommand{\prevq}{{\mymacro{ p }}}
\newcommand{\nextq}{{\mymacro{ n }}}
\newcommand{\weight}{{\mymacro{ \textnormal{w}}}}
\newcommand{\innerweight}{{\mymacro{ \weight_{\text{I}}}}}
\newcommand{\apath}{{\mymacro{ \boldsymbol \pi}}}
\newcommand{\pathlen}{{\mymacro{ N}}}
\newcommand{\paths}{{\mymacro{ \Pi}}}
\newcommand{\initial}{{\mymacro{ I}}}
\newcommand{\final}{{\mymacro{ F}}}
\newcommand{\initf}{{\mymacro{ \lambda}}}
\newcommand{\finalf}{{\mymacro{ \rho}}}
\newcommand{\initfFun}[1]{{\mymacro{\initf\left(#1\right)}}}
\newcommand{\finalfFun}[1]{{\mymacro{\finalf\left(#1\right)}}}
\newcommand{\initfVect}{{\mymacro{ \overrightarrow{\initf}}}}
\newcommand{\finalfVect}{{\mymacro{ \overrightarrow{\finalf}}}}
\newcommand{\qinit}{{\mymacro{ q_{\initial}}}}
\newcommand{\qfinal}{{\mymacro{ q_{\final}}}}
\newcommand{\sempty}{{\mymacro{ z_{\textit{0}}}}}
\newcommand{\strone}{{\mymacro{ \infty}}}
\newcommand{\strsemiring}{{\mymacro{ \mathcal{S}}}}
\newcommand{\kleenesemiring}{{\mymacro{ \mathcal{K}}}}
\newcommand{\transMtx}{{\mymacro{ \mT}}}
\newcommand{\allsum}{{\mymacro{ Z}}}
\newcommand{\pathsum}{{\mymacro{ \allsum}}}
\newcommand{\discover}[1]{{\mymacro{ d \left[ #1 \right]}}}
\newcommand{\finish}[1]{{\mymacro{ f \left[ #1 \right]}}}
\newcommand{\transitionWeight}{{\mymacro{ \omega}}}
\newcommand{\transitionWeightFun}[1]{{\mymacro{ \transitionWeight(#1)}}}

\newcommand{\fsatuple}{{\mymacro{ \left( \alphabet, \states, \initial, \final, \trans \right)}}}
\newcommand{\wfsatuple}{{\mymacro{ \left( \alphabet, \states, \trans, \initf, \finalf \right)}}}
\newcommand{\dfatuple}{{\mymacro{ \left( \alphabet, \states, \qinit, \final, \trans \right)}}}
\newcommand{\dist}[2]{{\mymacro{ d \left[ #1, #2 \right]}}}
\newcommand{\reverse}[1]{{\mymacro{ \overleftarrow{#1}}}}
\newcommand{\edgenoweight}[3]{#1 \xrightarrow{#2} #3}
\newcommand{\edge}[4]{{\mymacro{#1 \xrightarrow{#2 / #3} #4}}}
\newcommand{\uwedge}[3]{{\mymacro{#1 \xrightarrow{#2} #3}}}
\newcommand{\wfsttuple}{{\mymacro{ \left( \alphabet, \oalphabet, \states, \initial, \final, \trans, \initf, \finalf \right)}}}
\newcommand{\forwardweight}[1]{{\mymacro{ \boldsymbol{\alpha}_{#1}}}}
\newcommand{\backwardweight}[1]{{\mymacro{ \boldsymbol{\beta}_{#1}}}}
\newcommand{\distance}{{\mymacro{ \Delta}}}
\newcommand{\potentialfunction}{{\mymacro{ \Psi}}}
\newcommand{\powerstate}{{\mymacro{ \mathcal{Q}}}}
\newcommand{\initpowerstate}{{\mymacro{ \mathcal{Q}_{\initial}}}}
\newcommand{\mitr}[3]{{\mymacro{ #1_{#3}^{\left(#2\right)}}}}

\newcommand{\yield}{{\mymacro{\textbf{s}}}}
\newcommand{\arity}{{\mymacro{\textsf{arity}}}}
\newcommand{\topo}{{\mymacro{\textsf{topo}}}}
\newcommand{\rtopo}{{\mymacro{\textsf{rtopo}}}}
\newcommand{\copycmd}{{\mymacro{\textsf{copy}}}}
\newcommand{\tablefill}{{\mymacro{\textsf{table-filling}}}}

\newcommand{\partitionP}{{\mymacro{ \mathbf{\mathcal{P}}}}}
\newcommand{\partitionQ}{{\mymacro{ \mathbf{\mathcal{Q}}}}}
\newcommand{\partitionR}{{\mymacro{ \mathbf{\mathcal{R}}}}}
\newcommand{\partitionX}{{\mymacro{ \mathbf{\mathcal{X}}}}}
\newcommand{\refinementof}{{\mymacro{\preccurlyeq}}}
\newcommand{\refinementoff}{{\mymacro{ \preccurlyeq_f}}}
\newcommand{\refinementoffplus}{{\mymacro{ \preccurlyeq_f^+}}}
\newcommand{\splitpart}{{\mymacro{ \textsf{split}}}}
\newcommand{\splitpartfaster}{{\mymacro{ \textsf{split-modified}}}}
\newcommand{\finv}{{\mymacro{ f^{-1}}}}
\newcommand{\Requivalence}{{\mymacro{ R_{\lang}}}}
\newcommand{\eqclass}[1]{{\mymacro{ \left[#1\right]}}}
\newcommand{\nerodeeq}{{\mymacro{ \sim_{\lang}}}}
\newcommand{\stateeq}{{\mymacro{ \sim_{\trans}}}}

\newcommand{\fps}{{\mymacro{ r}}}
\newcommand{\fpscoef}[2]{{\mymacro{ #1_{#2}}}}
\newcommand{\fpss}{{\mymacro{ \semiring \langle \langle \kleene{\alphabet} \rangle \rangle}}}
\newcommand{\finitefpss}{{\mymacro{ \semiring \langle \kleene{\alphabet} \rangle}}}

\newcommand{\tm}{{\mymacro{ \mathcal{M}}}}
\newcommand{\ptmtuple}{\left(\states, \alphabet, \tapealphabet, \trans, \qinit, \qfinal \right)}
\newcommand{\ptmtupletwo}{\left(\states, \alphabet, \tapealphabet, \trans_1, \trans_2, \qinit, \qfinal \right)} %
\newcommand{\tapealphabet}{\mymacro{ \Gamma}}
\newcommand{\tmleft}{\mymacro{ L}}
\newcommand{\tmright}{\mymacro{ R}}
\newcommand{\blanksym}{\boldsymbol{\hash}}

\newcommand{\tsystem}{{\mymacro{ \mathcal{T}}}}
\newcommand{\tsystemstates}{{\mymacro{ S}}}
\newcommand{\tstate}{{\mymacro{ s}}}
\newcommand{\tstateInit}{{\mymacro{ \tstate_{\text{I}}}}}
\newcommand{\tstateu}{{\mymacro{ u}}}
\newcommand{\tsystemtuple}{{\mymacro{ \left(\alphabet, \tsystemstates, \dyMap, \tstateInit\right)}}}
\newcommand{\wtsystemtuple}{{\mymacro{ \left(\alphabet, \tsystemstates, \dyMap, \tstateInit\right)}}}
\newcommand{\observations}{{\mymacro{ \sO}}}
\newcommand{\observationmap}{{\mymacro{ o}}}
\newcommand{\dyMap}{{\mymacro{ \vfunc}}}
\newcommand{\generalrnntuple}{{\mymacro{ \left( \alphabet, \hiddDim, \dyMap, \hiddStateZero\right)}}}
\newcommand{\rnntuple}{{\mymacro{ \left( \alphabet, \hiddDim, \dyMap, \outMtx, \hiddStateZero\right)}}}
\newcommand{\elmanrnntuple}{{\mymacro{ \left( \alphabet, \sigmoid, \hiddDim, \recMtx, \inMtx, \biasVech, \hiddStateZero\right)}}}
\newcommand{\elmanUpdate}[2]{{\mymacro{ \sigmoid\left(\recMtx #1 + \inMtx \onehot{#2} + \biasVech\right)}}}
\newcommand{\rnn}{{\mymacro{ \mathcal{R}}}}
\newcommand{\rnnlm}{{\mymacro{\left(\rnn, \outMtx\right)}}}
\newcommand{\ernnAcr}{{\mymacro{ERNN}}}
\newcommand{\hernnAcr}{{\mymacro{HRNN}}}
\newcommand{\dpfsaAcr}{{\mymacro{DPFSA}}}
\newcommand{\recMtx}{{\mymacro{ \mU}}}
\newcommand{\inMtx}{{\mymacro{ \mV}}}
\newcommand{\outMtx}{{\mymacro{ \mE}}}
\newcommand{\eOutMtx}{{\mymacro{ \eembedMtx}}}
\newcommand{\eRecMtx}{{\mymacro{ \emU}}}
\newcommand{\eInMtx}{{\mymacro{ \emV}}}
\newcommand{\hiddDim}{{\mymacro{ D}}}
\newcommand{\Rhid}{{\mymacro{ \R^\hiddDim}}}
\newcommand{\gate}{{\mymacro{ \vg}}}
\newcommand{\gatet}{{\mymacro{ \gate_\tstep}}}

\newcommand{\hiddState}{{\mymacro{ \vh}}}
\newcommand{\hiddStatet}{{\mymacro{ \hiddState_\tstep}}}
\newcommand{\hiddStateT}{{\mymacro{ \hiddState_\strlen}}}
\newcommand{\hiddStateTminus}{{\mymacro{ \hiddState_{\strlen - 1}}}}
\newcommand{\hiddStatetplus}{{\mymacro{ \hiddState_{\tstep + 1}}}}
\newcommand{\hiddStatetminus}{{\mymacro{ \hiddState_{\tstep - 1}}}}
\newcommand{\context}{{\mymacro{ \vc}}}
\newcommand{\contextt}{{\mymacro{ \context_\tstep}}}
\newcommand{\vhzero}{{\mymacro{ \vh_0}}}
\newcommand{\vhone}{{\mymacro{ \vh_1}}}
\newcommand{\hiddStateZero}{{\mymacro{ \vhzero}}}
\newcommand{\hiddStateOne}{{\mymacro{ \vhone}}}
\newcommand{\vht}{{\mymacro{ \vh_t}}}
\newcommand{\vhZero}{{\mymacro{ \vh_0}}}
\newcommand{\vhi}{{\mymacro{ \vh_i}}}
\newcommand{\vhiminus}{{\mymacro{ \vh_{i-1}}}}
\newcommand{\vhT}{{\mymacro{ \vh_T}}}
\newcommand{\vhtminus}{{\mymacro{ \vh_{t-1}}}}
\newcommand{\vhTminus}{{\mymacro{ \vh_{T-1}}}}

\newcommand{\symordering}{{\mymacro{ m}}}
\newcommand{\eossymordering}{{\mymacro{\overline{\symordering}}}}
\newcommand{\stateordering}{{\mymacro{ r}}}
\newcommand{\anOrdering}{{\mymacro{ s}}}
\newcommand{\BtoQS}{{\mymacro{ \B^{|\states||\eosalphabet|}}}}
\newcommand{\BtoQSeos}{{\mymacro{ \B^{|\states||\eosalphabet|}}}}


\newcommand{\phiCoor}{{\mymacro{ \vvarphi}}}
\newcommand{\phitwo}{{\mymacro{ \phi_2}}}
\newcommand{\phifour}{{\mymacro{ \phi_4}}}
\newcommand{\phitwoFun}[1]{{\mymacro{ \phitwo\left(#1\right)}}}
\newcommand{\phifourFun}[1]{{\mymacro{ \phifour\left(#1\right)}}}
\newcommand{\phitwoInv}{{\mymacro{ \inv{\phi_2}}}}
\newcommand{\phifourInv}{{\mymacro{ \inv{\phi_4}}}}
\newcommand{\phitwoInvFun}[1]{{\mymacro{ \phitwoInv\left(#1\right)}}}
\newcommand{\phifourInvFun}[1]{{\mymacro{ \phifourInv\left(#1\right)}}}
\newcommand{\project}[1]{{\mymacro{ \pi_{#1}}}}
\newcommand{\nfs}{{\mymacro{ C}}}
\newcommand{\srNstates}{{\mymacro{ s}}}
\newcommand{\frNstates}{{\mymacro{ r}}}
\newcommand{\BQQ}{{\mymacro{ \B^{\nstates \times \nstates}}}}
\newcommand{\BtwoQ}{{\mymacro{ \B^{2 \nstates}}}}
\newcommand{\Bss}{{\mymacro{ \B^{\srNstates \times \srNstates}}}}
\newcommand{\Btwos}{{\mymacro{ \B^{2 \srNstates}}}}
\newcommand{\qvectv}[1]{{\mymacro{ \vv\left(#1\right)}}}
\newcommand{\qvectu}[1]{{\mymacro{ \vu\left(#1\right)}}}
\newcommand{\qBs}[1]{{\mymacro{ \sB\left(#1\right)}}}
\newcommand{\stateSet}{{\mymacro{ \mathcal{Q}}}}
\newcommand{\qPreds}[1]{{\mymacro{ \texttt{Par}\left(#1\right)}}}
\newcommand{\qt}{{\mymacro{ \stateq_\tstep}}}
\newcommand{\qT}{{\mymacro{ \stateq_\strlen}}}
\newcommand{\qTminus}{{\mymacro{ \stateq_\strlen}}}
\newcommand{\qtminus}{{\mymacro{ \stateq_{\tstep - 1}}}}
\newcommand{\qtplus}{{\mymacro{ \stateq_{\tstep + 1}}}}
\newcommand{\balpha}{{\mymacro{ \boldsymbol{\alpha}}}}
\newcommand{\nLines}[1]{{\mymacro{ L\left(#1\right)}}}
\newcommand{\compMtx}[2]{{\mymacro{ \Phi_{#1, #2}}}}
\newcommand{\sepwfsa}{{\mymacro{ \wfsa_{\alphabet}}}}


\newcommand{\grammar}{{\mymacro{ \mathcal{G}}}}
\newcommand{\nonterm}{{\mymacro{ \mathcal{N}}}}
\newcommand{\rules}{{\mymacro{ \mathcal{P}}}}
\newcommand{\arule}{{\mymacro{ p}}}
\newcommand{\cfgstr}{{\mymacro{ \valpha}}} %
\newcommand{\start}{{\mymacro{ \NT{S}}}}
\newcommand{\cfgtuple}{{\mymacro{ \left(\alphabet, \nonterm, \start, \rules \right)}}}
\newcommand{\derivationset}[2]{{\mymacro{ \mathcal{D}_{#1}(#2)}}}
\newcommand{\grammarDerivationset}[1]{{\mymacro{ \mathcal{D}_{#1}}}}
\newcommand{\tree}{{\mymacro{\boldsymbol{d}}}}
\newcommand{\treeyield}[1]{{\mymacro{ \str(#1)}}}
\newcommand{\production}[2]{{\mymacro{ #1 \rightarrow #2}}}
\newcommand{\wproduction}[3]{{\mymacro{ #1 \xrightarrow {#3} #2}}}
\newcommand{\derives}{{\mymacro{ \overset{*}{\Rightarrow}}}}
\newcommand{\derivesbase}{{\mymacro{ \Rightarrow}}}
\newcommand{\wcfgtuple}{(\alphabet, \nonterm, \start, \rules, \productionWeight)}
\newcommand{\desc}[1]{\textsf{descendant}(#1)}
\newcommand{\children}[1]{\textsf{children}(#1)}
\newcommand{\depth}[1]{\textsf{depth}(#1)}
\newcommand{\height}[1]{\textsf{height}(#1)}
\newcommand{\property}{{\mymacro{ P}}}
\newcommand{\class}{{\mymacro{ \mathcal C}}}
\newcommand{\treeroot}{{\mymacro{ \rho}}}
\newcommand{\NT}[1]{{\mymacro{ \mathrm{#1}}}}
\newcommand{\NTA}{\NT{A}}
\newcommand{\NTB}{\NT{B}}
\newcommand{\NTC}{\NT{C}}
\newcommand{\NTX}{\NT{X}}
\newcommand{\NTY}{\NT{Y}}
\newcommand{\NTZ}{\NT{Z}}
\newcommand{\transform}{{\mymacro{ \mathcal{T}}}}
\newcommand{\productionWeight}{{\mymacro{ \mathcal{W}}}}
\newcommand{\genFunc}{{\mymacro{ G}}}

\newcommand{\emb}{{\mymacro{\mathsf{emb}}}}
\newcommand{\embfunc}[1]{{\mymacro{\mathsf{emb}}} (#1)}
\newcommand{\enc}{{\mymacro{\mathsf{enc}}}}
\newcommand{\encfunc}[1]{{\mymacro{\mathsf{enc}}} (#1)}
\newcommand{\encRNN}{\mymacro{\mathsf{enc}_{\rnn}}}
\newcommand{\encRNNfunc}[1]{\mymacro{ \encRNN\!\left(#1\right)}}
\newcommand{\mlp}{{\mymacro{\mathsf{MLP}}}}
\newcommand{\simplexFun}[1]{{\mymacro{ \boldsymbol{\Delta}}^{#1}}}
\newcommand{\Simplexd}{{\mymacro{ \boldsymbol{\Delta}^D}}}
\newcommand{\Simplexdminus}{{\mymacro{ \boldsymbol{\Delta}^{D-1}}}}
\newcommand{\Simplexalphabetminus}{{\mymacro{ \boldsymbol{\Delta}^{|\eosalphabet|-1}}}}
\newcommand{\SimplexEosalphabetminus}{{\mymacro{ \boldsymbol{\Delta}^{|\eosalphabet|-1}}}}
\newcommand{\ent}{{\mymacro{\mathrm{H}}}}

\newcommand{\locPar}{{\mymacro{k}}}


\newcommand{\mtxDim}{{\mymacro{ N}}}
\newcommand{\spectRad}{{\mymacro{ \rho_{\text{s}}}}}



\let\rfb\reflectbox
\newcommand{\uglyfrac}[2]{\rfb{\nicefrac{\rfb{#1}}{\ \rfb{#2}}}}
\newcommand{\lc}[2]{{\mymacro{ #1\mathtosmaller{\setminus}#2 }}}
\newcommand{\negterm}[1]{{\mymacro{ {\raise.17ex\hbox{$\scriptstyle\sim$}} #1}}}
\newcommand{\lcrules}{{\mymacro{ \rules_{\mathtosmaller{\setminus}}}}}
\newcommand{\lcnonterm}{{\mymacro{ \nonterm_{\mathtosmaller{\setminus}}}}}
\newcommand{\lcmap}{{\mymacro{ \mu}}}

\newcommand{\ifcondition}{\textbf{if }}
\newcommand{\otherwisecondition}{\textbf{otherwise }}
\newcommand{\algoName}[1]{{\mymacro{\textsc{#1}}}}
\newcommand{\forward}{{\mymacro{ \text{forward}}}}
\newcommand{\backward}{{\mymacro{ \text{backward}}}}
\newcommand{\pathsumAlg}{{\mymacro{ \text{pathsum}}}}
\newcommand{\viterbi}{{\mymacro{ \text{Viterbi}}}}
\newcommand{\dijkstra}{{\mymacro{ \text{Dijkstra}}}}
\newcommand{\fixedpoint}{{\mymacro{ \text{FixedPoint}}}}
\newcommand{\gaussjordan}{{\mymacro{ \text{GaussJordan}}}}
\newcommand{\floydwarshall}{{\mymacro{ \text{FloydWarshall}}}}
\newcommand{\bellmanford}{{\mymacro{ \text{BellmanFord}}}}
\newcommand{\gaussjordandiff}{{\mymacro{ \text{GaussJordanDifference}}}}
\newcommand{\determinization}{{\mymacro{ \text{Determinize}}}}
\newcommand{\moore}{{\mymacro{ \text{Moore}}}}
\newcommand{\minconstruction}{{\mymacro{ \text{BlockFSAConstruction}}}}
\newcommand{\partitionrefinement}{{\mymacro{ \text{PartitionRefinement}}}}
\newcommand{\naivepartitionrefinement}{{\mymacro{ \text{Na{\"i}vePartitionRefinement}}}}
\newcommand{\moorepartition}{{\mymacro{ \text{MoorePartition}}}}
\newcommand{\hopcroft}{{\mymacro{ \text{Hopcroft}}}}
\newcommand{\hopcroftfast}{{\mymacro{ \text{FastHopcroft}}}}
\newcommand{\partitionminimization}{{\mymacro{ \text{PartitionRefinementMinimization}}}}
\newcommand{\weighteddeterminization}{{\mymacro{ \text{WeightedDeterminize}}}}
\newcommand{\naiveintersection}{{\mymacro{ \text{Na{\"i}veIntersect}}}}
\newcommand{\filteredintersection}{{\mymacro{ \text{$\epsilon$-filterIntersect}}}}
\newcommand{\intersection}{{\mymacro{ \text{Intersect}}}}
\newcommand{\lehmann}{{\mymacro{ \text{Lehmann}}}}
\newcommand{\decomposedlehmann}{{\mymacro{ \text{DecomposedLehmann}}}}
\newcommand{\sccfsa}{{\mymacro{ \text{SccFsa}}}}
\newcommand{\dfs}{{\mymacro{ \text{DepthFirstSearch}}}}
\newcommand{\toposort}{{\mymacro{ \text{TopologicalSort}}}}
\newcommand{\dfsrec}{{\mymacro{ \text{DepthFirstSearchRecursion}}}}
\newcommand{\kosaraju}{{\mymacro{ \text{Kosaraju}}}}
\newcommand{\accessibility}{{\mymacro{ \text{Accessible}}}}
\newcommand{\trim}{{\mymacro{ \text{Trim}}}}
\newcommand{\testtwins}{{\mymacro{ \text{TestTwinsProperty}}}}
\newcommand{\acyclicwcfg}{{\mymacro{ \text{AcyclicTreesum}}}}
\newcommand{\fixedpointcfg}{{\mymacro{ \text{FixedPointGrammar}}}}
\newcommand{\cycleidentity}{{\mymacro{ \text{CycleIdentity}}}}
\newcommand{\acceptance}{{\mymacro{ \text{Acceptance}}}}
\newcommand{\epsremoval}{{\mymacro{ \varepsilon\text{-}\text{removal}}}}
\newcommand{\weightpushing}{{\mymacro{ WeightPush}}}
\newcommand{\unweightedminimization}{{\mymacro{ \text{UnweightedMinimization}}}}
\newcommand{\separateunks}{{\mymacro{ \text{Separateunks}}}}
\newcommand{\nullaryremoval}{{\mymacro{ \text{RemoveNullary}}}}
\newcommand{\makeunarywfsa}{{\mymacro{ \text{MakeUnaryWFSA}}}}
\newcommand{\wfsatowcfg}{{\mymacro{ \text{WeightedAutomatonConversion}}}}
\newcommand{\unaryremoval}{{\mymacro{ \text{RemoveUnary}}}}
\newcommand{\trimcfg}{{\mymacro{ \text{TrimCFG}}}}
\newcommand{\weightedunfold}{{\mymacro{ \text{WeightedUnfold}}}}
\newcommand{\weightedfold}{{\mymacro{ \text{WeightedFold}}}}
\newcommand{\binarize}{{\mymacro{ \text{Binarize}}}}
\newcommand{\union}{{\mymacro{ \text{Union}}}}
\newcommand{\complementation}{{\mymacro{ \text{Complementation}}}}
\newcommand{\separationAlgoName}{{\algoName{Separate}}}




\newcommand{\pdatuple}{\left(\states, \alphabet,  \stackalphabet, \trans, \pdaconfig{\initstack}{\qinit}, \pdaconfig{\finalstack}{\qfinal}\right)}
\newcommand{\wpdatuple}{\left(\states, \alphabet, \stackalphabet, \trans, \pdaconfig{\initstack}{\qinit}, \pdaconfig{\finalstack}{\qfinal} \right)}
\newcommand{\twostackpdatuple}{\left(\states, \alphabet, \stackalphabet, \trans, \pdaconfig{\initstack,\initstacktwo}{\qinit}, \pdaconfig{\finalstack,\finalstacktwo}{\qfinal}\right)}
\newcommand{\twostackwpdatuple}{\left(\states, \alphabet, \stackalphabet, \trans , \pdaconfig{\initstack,\initstacktwo}{\qinit}, \pdaconfig{\finalstack,\finalstacktwo}{\qfinal} \right)}
\newcommand{\twostackgppdatuple}{\left(\states, \alphabet, \stackalphabet, \trans_1, \trans_2, \qinit, \qfinal \right)} %
\newcommand{\pdatupleNorm}{\left( \states, \alphabet, \stackalphabet, \qinit, \sempty, \qfinal, \trans  \right)}
\newcommand{\pushdown}{\mymacro{ \mathcal{P}}}
\newcommand{\pda}{\mymacro{ \pushdown}}
\newcommand{\bottomup}{\mymacro{ \textsf{bottomup}}}
\newcommand{\topdown}{\mymacro{ \textsf{topdown}}}
\newcommand{\shift}{\textsc{shift}}
\newcommand{\reduce}{\textsc{reduce}}
\newcommand{\pdaEdge}[6]{\mymacro{ \edge{#2}{#3, #5 \rightarrow #6}{#1}{#4}}}
\newcommand{\twoPdaEdge}[8]{\mymacro{ \edge{#2}{#3, #5 \rightarrow #6, #7 \rightarrow #8}{#1}{#4}}}
\newcommand{\pdaEdgenoweight}[5]{{\mymacro{ \edgenoweight{#1}{#2, #4 \rightarrow #5}{#3}}}}
\newcommand{\arun}{{\mymacro{ \apath}}}
\newcommand{\runs}{{\mymacro{ \paths}}}
\newcommand{\stackseq}{{\mymacro{ {\boldsymbol{\gamma}}}}}
\newcommand{\stackseqtwo}{{\mymacro{ {\boldsymbol{\sigma}}}}}
\newcommand{\emptystack}{{\mymacro{ {\emptyset}}}}
\newcommand{\initstack}{{\mymacro{ {\stackseq_{\initial}}}}}
\newcommand{\finalstack}{{\mymacro{ {\stackseq_{\final}}}}}
\newcommand{\initstacktwo}{{\mymacro{ {\stackseqtwo_{\initial}}}}}
\newcommand{\finalstacktwo}{{\mymacro{ {\stackseqtwo_{\final}}}}}
\newcommand{\pdaconfig}[2]{{\mymacro{ \left(#2, #1\right)}}}
\newcommand{\twoPdaconfig}[3]{{\mymacro{ \left(#3, #1, #2\right)}}}
\newcommand{\prevs}[1]{{\mymacro{ W_q \left( #1 \right) }}}
\newcommand{\nexts}[1]{{\mymacro{ W_n \left( #1 \right) }}}
\newcommand{\stacksymbol}[1]{{\mymacro{ #1 }}}
\newcommand{\transweight}[5]{
    {\mymacro{ \trans(#1,\stacksymbol{#4}\xrightarrow{#2}#3,\stacksymbol{#5})}}}
\newcommand{\atrans}{{\mymacro{ \tau}}}
\newcommand{\pdaAction}{{\mymacro{ a}}}
\newcommand{\pushOp}{{\mymacro{ \texttt{PUSH}}}}
\newcommand{\popOp}{{\mymacro{ \texttt{POP}}}}
\newcommand{\noOp}{{\mymacro{ \texttt{NO-OP}}}}
\newcommand{\peekOp}{{\mymacro{ \texttt{PEEK}}}}

\newcommand{\stackCell}{{\mymacro{ \texttt{STACK}}}}
\newcommand{\rnnPhase}[1]{{\mymacro{ \texttt{PHASE}_{#1}}}}
\newcommand{\bufferCell}[1]{{\mymacro{ \texttt{BUFF}_{#1}}}}
\newcommand{\acceptCell}{{\mymacro{ \texttt{ACCEPT}}}}
\newcommand{\stackTopCell}[1]{{\mymacro{ \texttt{STACK}_{#1}}}}
\newcommand{\stackTopCellEmpty}{{\mymacro{ \texttt{STACK}_{\eps}}}}
\newcommand{\stackTopCellZero}{{\mymacro{ \texttt{STACK}_{0}}}}
\newcommand{\stackTopCellOne}{{\mymacro{ \texttt{STACK}_{1}}}}
\newcommand{\stackInputConfig}[2]{{\mymacro{ \texttt{CONF}_{#1, #2}}}}
\newcommand{\stackComp}[2]{{\mymacro{ \texttt{OP}_{#1, #2}}}}
\newcommand{\stackCompNoOp}{{\mymacro{ \texttt{OP}_{\noOp}}}}
\newcommand{\stackToNumeric}[1]{{\mymacro{ \texttt{rep}\left(#1\right)}}}
\newcommand{\stackSymToDigit}[1]{{\mymacro{ \texttt{digit}\left(#1\right)}}}


\newcommand{\curlyarrow}{{\mymacro{ \mathrel{\leadsto}}}}

\newcommand{\ignore}[1]{}
\newcommand{\expandLater}[1]{}

\newcommand{\tfslen}{\mymacro{\finaltstep}}
\newcommand{\tfheadnum}{\mymacro{H}}

\newcommand{\qTransf}{\mymacro{Q}}
\newcommand{\kTransf}{\mymacro{K}}
\newcommand{\vTransf}{\mymacro{V}}
\newcommand{\oTransf}{\mymacro{O}}
\newcommand{\fTransf}{\mymacro{F}}
\newcommand{\qTransfFun}[1]{\mymacro{\qTransf\left(#1\right)}}
\newcommand{\kTransfFun}[1]{\mymacro{\kTransf\left(#1\right)}}
\newcommand{\vTransfFun}[1]{\mymacro{\vTransf\left(#1\right)}}
\newcommand{\oTransfFun}[1]{\mymacro{\oTransf\left(#1\right)}}
\newcommand{\fTransfFun}[1]{\mymacro{\fTransf\left(#1\right)}}

\newcommand{\qMtx}{\mymacro{\mW_Q}}
\newcommand{\kMtx}{\mymacro{\mW_K}}
\newcommand{\vMtx}{\mymacro{\mW_V}}

\newcommand{\attn}{\mymacro{\texttt{Att}}}
\newcommand{\attnBlock}{\mymacro{\texttt{A}}}
\newcommand{\attnBlockMH}{\mymacro{\tflayer^\tfheadnum}}
\newcommand{\attnfunc}{\mymacro{\vfunc_\texttt{Att}}}
\newcommand{\tfheadCombine}{\mymacro{\mathcal{H}}}

\newcommand{\transformernetwork}{\mymacro{\mathcal{T}}}
\newcommand{\tf}{\mymacro{\mathcal{T}}}
\newcommand{\tfFun}[1]{\tf\left(#1\right)}
\newcommand{\tfpLM}{\mymacro{\pLM_\transformernetwork}}
\newcommand{\tfencfun}{\mymacro{\enc}}
\newcommand{\transformertuple}{\mymacro{(\alphabet, \hiddDim, \tfencfun)}}
\newcommand{\tfseqmodel}{\mymacro{(\alphabet, \hiddDim, \tfencfun, \embedMtx)}}
\newcommand{\tfLipfunc}{\mymacro{\vfunc^\tstep_\tf}}

\newcommand{\idfun}{\mymacro{\text{Id}}}

\newcommand{\tfscorefun}{\mymacro{\func}}
\newcommand{\tfembfun}{\mymacro{\vr}}
\newcommand{\hardmax}{\mymacro{\mathrm{hardmax}}}
\newcommand{\hardmaxAvg}{\mymacro{\hardmax}}
\newcommand{\hardmaxUni}{\mymacro{\hardmax_\textnormal{uni}}}

\newcommand{\tflayer}{\mymacro{\mathrm{\mathcal{L}}}}
\newcommand{\tflayerinputmat}{\mymacro{\mX}}
\newcommand{\tflayerinputsy}{\mymacro{\vx}}
\newcommand{\tflayerinputseq}{\mymacro{(\tflayerinputsy^\top_1; \cdots;  \tflayerinputsy^\top_\tfslen)}}
\newcommand{\tflayeroutputmat}{\mymacro{\mZ}}
\newcommand{\tflayeroutputsy}{\mymacro{\vz}}
\newcommand{\tflayeroutputseq}{\mymacro{(\tflayeroutputsy^\top_1; \cdots;  \tflayeroutputsy^\top_\tfslen)}}
\newcommand{\tflayeridx}{\mymacro{\ell}}
\newcommand{\tfnumlayer}{\mymacro{L}}
\newcommand{\tfencnumlayer}{\mymacro{\tfnumlayer_{\mathrm{enc}}}}
\newcommand{\tfdecnumlayer}{\mymacro{\tfnumlayer_{\mathrm{dec}}}}
\newcommand{\posEnc}{\mymacro{\Pi}}
\newcommand{\absPosEnc}{\mymacro{\posEnc_{\texttt{A}}}}
\newcommand{\relEncLen}{\mymacro{r}}
\newcommand{\relPosEnc}{\mymacro{\posEnc_{\texttt{R}}}}
\newcommand{\posEncFun}[1]{\mymacro{\posEnc\left(#1\right)}}
\newcommand{\relPosEncFun}[1]{\mymacro{\relPosEnc\left(#1\right)}}
\newcommand{\absPosEncFun}[1]{\mymacro{\absPosEnc\left(#1\right)}}
\newcommand{\posInEmbedding}{\mymacro{\inEmbedding_{\scaleto{\posEnc}{4pt}}}}
\newcommand{\posInEmbeddingFun}[1]{\mymacro{\posInEmbedding\left(#1\right)}}

\newcommand{\layerNorm}{\mymacro{\texttt{LN}}}
\newcommand{\layerNormFun}[1]{\mymacro{\layerNorm\left(#1\right)}}

\newcommand{\headqkvparams}{\mymacro{\boldsymbol{\mathcal{W}}_{qkv}}}
\newcommand{\ffnparams}{\mymacro{\boldsymbol{\mathcal{W}}^{\textnormal{FFN}}}}
\newcommand{\multiheadparams}{\mymacro{\boldsymbol{\mathcal{W}}^{\textnormal{MH}}}}
\newcommand{\actfn}[1]{\mymacro{\boldsymbol{\phi}(#1)}}


\newcommand{\extAlphabet}{{\mymacro{ \Delta}}}
\newcommand{\actionToNum}[1]{{\mymacro{ \texttt{d}\left(#1\right)}}}

\newcommand{\kernel}[2]{{\mymacro{ K(#1, #2)}}}
\newcommand{\gkernel}[2]{{\mymacro{ K_{\mathrm{G}}(#1, #2)}}}
\newcommand{\smkernel}[2]{{\mymacro{ K_{\mathrm{SM}}(#1, #2)}}}





\def\bw{{{\mymacro{ \textbf{w}}}}}


\def\1{\mathbf{1}}
\newcommand{\dataset}{{\mymacro{\mathcal{D}}}}
\newcommand{\train}{{\mymacro{\mathcal{D_{\mathrm{valid}}}}}}
\newcommand{\valid}{{\mymacro{\mathcal{D_{\mathrm{valid}}}}}}
\newcommand{\test}{{\mymacro{\mathcal{D_{\mathrm{test}}}}}}

\def\eps{{\mymacro{ \varepsilon}}}


\def\reta{{{\mymacro{ \textnormal{\eta}}}}}
\def\ra{{{\mymacro{ \textnormal{a}}}}}
\def\rb{{{\mymacro{ \textnormal{b}}}}}
\def\rc{{{\mymacro{ \textnormal{c}}}}}
\def\rd{{{\mymacro{ \textnormal{d}}}}}
\def\re{{{\mymacro{ \textnormal{e}}}}}
\def\rf{{{\mymacro{ \textnormal{f}}}}}
\def\rg{{{\mymacro{ \textnormal{g}}}}}
\def\rh{{{\mymacro{ \textnormal{h}}}}}
\def\ri{{{\mymacro{ \textnormal{i}}}}}
\def\rj{{{\mymacro{ \textnormal{j}}}}}
\def\rk{{{\mymacro{ \textnormal{k}}}}}
\def\rl{{{\mymacro{ \textnormal{l}}}}}
\def\rn{{{\mymacro{ \textnormal{n}}}}}
\def\ro{{{\mymacro{ \textnormal{o}}}}}
\def\rp{{{\mymacro{ \textnormal{p}}}}}
\def\rq{{{\mymacro{ \textnormal{q}}}}}
\def\rr{{{\mymacro{ \textnormal{r}}}}}
\def\rs{{{\mymacro{ \textnormal{s}}}}}
\def\rt{{{\mymacro{ \textnormal{t}}}}}
\def\ru{{{\mymacro{ \textnormal{u}}}}}
\def\rv{{{\mymacro{ \textnormal{v}}}}}
\def\rw{{{\mymacro{ \textnormal{w}}}}}
\def\rx{{{\mymacro{ \textnormal{x}}}}}
\def\ry{{{\mymacro{ \textnormal{y}}}}}
\def\rz{{{\mymacro{ \textnormal{z}}}}}
\def\reps{{{\mymacro{ \eps}}}}

\def\rvepsilon{{{\mymacro{ \boldsymbol{\epsilon}}}}}
\def\rvtheta{{{\mymacro{ \boldsymbol{\theta}}}}}
\def\rva{{{\mymacro{ \mathbf{a}}}}}
\def\rvb{{{\mymacro{ \mathbf{b}}}}}
\def\rvc{{{\mymacro{ \mathbf{c}}}}}
\def\rvd{{{\mymacro{ \mathbf{d}}}}}
\def\rve{{{\mymacro{ \mathbf{e}}}}}
\def\rvf{{{\mymacro{ \mathbf{f}}}}}
\def\rvg{{{\mymacro{ \mathbf{g}}}}}
\def\rvh{{{\mymacro{ \mathbf{h}}}}}
\def\rvu{{{\mymacro{ \mathbf{i}}}}}
\def\rvj{{{\mymacro{ \mathbf{j}}}}}
\def\rvk{{{\mymacro{ \mathbf{k}}}}}
\def\rvl{{{\mymacro{ \mathbf{l}}}}}
\def\rvm{{{\mymacro{ \mathbf{m}}}}}
\def\rvn{{{\mymacro{ \mathbf{n}}}}}
\def\rvo{{{\mymacro{ \mathbf{o}}}}}
\def\rvp{{{\mymacro{ \mathbf{p}}}}}
\def\rvq{{{\mymacro{ \mathbf{q}}}}}
\def\rvr{{{\mymacro{ \mathbf{r}}}}}
\def\rvs{{{\mymacro{ \mathbf{s}}}}}
\def\rvt{{{\mymacro{ \mathbf{t}}}}}
\def\rvu{{{\mymacro{ \mathbf{u}}}}}
\def\rvv{{{\mymacro{ \mathbf{v}}}}}
\def\rvw{{{\mymacro{ \mathbf{w}}}}}
\def\rvx{{{\mymacro{ \mathbf{x}}}}}
\def\rvy{{{\mymacro{ \mathbf{y}}}}}
\def\rvz{{{\mymacro{ \mathbf{z}}}}}
\def\rveps{{{\mymacro{ \boldsymbol{\reps}}}}}

\def\erva{{{\mymacro{ \textnormal{a}}}}}
\def\ervb{{{\mymacro{ \textnormal{b}}}}}
\def\ervc{{{\mymacro{ \textnormal{c}}}}}
\def\ervd{{{\mymacro{ \textnormal{d}}}}}
\def\erve{{{\mymacro{ \textnormal{e}}}}}
\def\ervf{{{\mymacro{ \textnormal{f}}}}}
\def\ervg{{{\mymacro{ \textnormal{g}}}}}
\def\ervh{{{\mymacro{ \textnormal{h}}}}}
\def\ervi{{{\mymacro{ \textnormal{i}}}}}
\def\ervj{{{\mymacro{ \textnormal{j}}}}}
\def\ervk{{{\mymacro{ \textnormal{k}}}}}
\def\ervl{{{\mymacro{ \textnormal{l}}}}}
\def\ervm{{{\mymacro{ \textnormal{m}}}}}
\def\ervn{{{\mymacro{ \textnormal{n}}}}}
\def\ervo{{{\mymacro{ \textnormal{o}}}}}
\def\ervp{{{\mymacro{ \textnormal{p}}}}}
\def\ervq{{{\mymacro{ \textnormal{q}}}}}
\def\ervr{{{\mymacro{ \textnormal{r}}}}}
\def\ervs{{{\mymacro{ \textnormal{s}}}}}
\def\ervt{{{\mymacro{ \textnormal{t}}}}}
\def\ervu{{{\mymacro{ \textnormal{u}}}}}
\def\ervv{{{\mymacro{ \textnormal{v}}}}}
\def\ervw{{{\mymacro{ \textnormal{w}}}}}
\def\ervx{{{\mymacro{ \textnormal{x}}}}}
\def\ervy{{{\mymacro{ \textnormal{y}}}}}
\def\ervz{{{\mymacro{ \textnormal{z}}}}}

\def\rmA{{{\mymacro{ \mathbf{A}}}}}
\def\rmB{{{\mymacro{ \mathbf{B}}}}}
\def\rmC{{{\mymacro{ \mathbf{C}}}}}
\def\rmD{{{\mymacro{ \mathbf{D}}}}}
\def\rmE{{{\mymacro{ \mathbf{E}}}}}
\def\rmF{{{\mymacro{ \mathbf{F}}}}}
\def\rmG{{{\mymacro{ \mathbf{G}}}}}
\def\rmH{{{\hiddmacro{ \mathbf{H}}}}}
\def\rmI{{{\mymacro{ \mathbf{I}}}}}
\def\rmJ{{{\mymacro{ \mathbf{J}}}}}
\def\rmK{{{\mymacro{ \mathbf{K}}}}}
\def\rmL{{{\mymacro{ \mathbf{L}}}}}
\def\rmM{{{\mymacro{ \mathbf{M}}}}}
\def\rmN{{{\mymacro{ \mathbf{N}}}}}
\def\rmO{{{\mymacro{ \mathbf{O}}}}}
\def\rmP{{{\mymacro{ \mathbf{P}}}}}
\def\rmQ{{{\mymacro{ \mathbf{Q}}}}}
\def\rmR{{{\mymacro{ \mathbf{R}}}}}
\def\rmS{{{\mymacro{ \mathbf{S}}}}}
\def\rmT{{{\mymacro{ \mathbf{T}}}}}
\def\rmU{{{\mymacro{ \mathbf{U}}}}}
\def\rmV{{{\mymacro{ \mathbf{V}}}}}
\def\rmW{{{\mymacro{ \mathbf{W}}}}}
\def\rmX{{{\mymacro{ \mathbf{X}}}}}
\def\rmY{{{\mymacro{ \mathbf{Y}}}}}
\def\rmZ{{{\mymacro{ \mathbf{Z}}}}}

\def\ermA{{{\mymacro{ \textnormal{A}}}}}
\def\ermB{{{\mymacro{ \textnormal{B}}}}}
\def\ermC{{{\mymacro{ \textnormal{C}}}}}
\def\ermD{{{\mymacro{ \textnormal{D}}}}}
\def\ermE{{{\mymacro{ \textnormal{E}}}}}
\def\ermF{{{\mymacro{ \textnormal{F}}}}}
\def\ermG{{{\mymacro{ \textnormal{G}}}}}
\def\ermH{{{\mymacro{ \textnormal{H}}}}}
\def\ermI{{{\mymacro{ \textnormal{I}}}}}
\def\ermJ{{{\mymacro{ \textnormal{J}}}}}
\def\ermK{{{\mymacro{ \textnormal{K}}}}}
\def\ermL{{{\mymacro{ \textnormal{L}}}}}
\def\ermM{{{\mymacro{ \textnormal{M}}}}}
\def\ermN{{{\mymacro{ \textnormal{N}}}}}
\def\ermO{{{\mymacro{ \textnormal{O}}}}}
\def\ermP{{{\mymacro{ \textnormal{P}}}}}
\def\ermQ{{{\mymacro{ \textnormal{Q}}}}}
\def\ermR{{{\mymacro{ \textnormal{R}}}}}
\def\ermS{{{\mymacro{ \textnormal{S}}}}}
\def\ermT{{{\mymacro{ \textnormal{T}}}}}
\def\ermU{{{\mymacro{ \textnormal{U}}}}}
\def\ermV{{{\mymacro{ \textnormal{V}}}}}
\def\ermW{{{\mymacro{ \textnormal{W}}}}}
\def\ermX{{{\mymacro{ \textnormal{X}}}}}
\def\ermY{{{\mymacro{ \textnormal{Y}}}}}
\def\ermZ{{{\mymacro{ \textnormal{Z}}}}}

\def\vzero{{{\mymacro{ \mathbf{0}}}}}
\def\vone{{{\mymacro{ \mathbf{1}}}}}
\def\vmu{{{\mymacro{ \boldsymbol{\mu}}}}}
\def\vtheta{{{\mymacro{ \boldsymbol{\theta}}}}}
\def\vphi{{{\mymacro{ \boldsymbol{\phi}}}}}
\def\vvarphi{{{\mymacro{ \boldsymbol{\varphi}}}}}
\def\va{{{\mymacro{ \mathbf{a}}}}}
\def\vb{{{\mymacro{ \mathbf{b}}}}}
\def\vc{{{\mymacro{ \mathbf{c}}}}}
\def\vd{{{\mymacro{ \mathbf{d}}}}}
\def\ve{{{\mymacro{ \mathbf{e}}}}}
\def\vf{{{\mymacro{ \mathbf{f}}}}}
\def\vg{{{\mymacro{ \mathbf{g}}}}}
\def\vh{{{\hiddmacro{ \mathbf{h}}}}}
\def\vi{{{\mymacro{ \mathbf{i}}}}}
\def\vj{{{\mymacro{ \mathbf{j}}}}}
\def\vk{{{\mymacro{ \mathbf{k}}}}}
\def\vl{{{\mymacro{ \mathbf{l}}}}}
\def\vm{{{\mymacro{ \mathbf{m}}}}}
\def\vn{{{\mymacro{ \mathbf{n}}}}}
\def\vo{{{\mymacro{ \mathbf{o}}}}}
\def\vp{{{\mymacro{ \mathbf{p}}}}}
\def\vq{{{\mymacro{ \mathbf{q}}}}}
\def\vr{{{\mymacro{ \mathbf{r}}}}}
\def\vs{{{\mymacro{ \mathbf{s}}}}}
\def\vt{{{\mymacro{ \mathbf{t}}}}}
\def\vu{{{\mymacro{ \mathbf{u}}}}}
\def\vv{{{\mymacro{ \mathbf{v}}}}}
\def\vw{{{\mymacro{ \mathbf{w}}}}}
\def\vx{{{\mymacro{ \mathbf{x}}}}}
\def\vy{{{\mymacro{ \mathbf{y}}}}}
\def\vz{{{\mymacro{ \mathbf{z}}}}}

\def\evalpha{{{\mymacro{ \alpha}}}}
\def\eveta{{{\mymacro{ \eta}}}}
\def\evlambda{{{\mymacro{ \lambda}}}}
\def\evbeta{{{\mymacro{ \beta}}}}
\def\evepsilon{{{\mymacro{ \epsilon}}}}
\def\evlambda{{{\mymacro{ \lambda}}}}
\def\evomega{{{\mymacro{ \omega}}}}
\def\evmu{{{\mymacro{ \mu}}}}
\def\evvarphi{{{\mymacro{ \varphi}}}}
\def\evpsi{{{\mymacro{ \psi}}}}
\def\evsigma{{{\mymacro{ \sigma}}}}
\def\evtheta{{{\mymacro{ \theta}}}}
\def\eva{{{\mymacro{ a}}}}
\def\evb{{{\mymacro{ b}}}}
\def\evc{{{\mymacro{ c}}}}
\def\evd{{{\mymacro{ d}}}}
\def\eve{{{\mymacro{ e}}}}
\def\evf{{{\mymacro{ f}}}}
\def\evg{{{\mymacro{ g}}}}
\def\evh{{{\mymacro{ h}}}}
\def\evi{{{\mymacro{ i}}}}
\def\evj{{{\mymacro{ j}}}}
\def\evk{{{\mymacro{ k}}}}
\def\evl{{{\mymacro{ l}}}}
\def\evm{{{\mymacro{ m}}}}
\def\evn{{{\mymacro{ n}}}}
\def\evo{{{\mymacro{ o}}}}
\def\evp{{{\mymacro{ p}}}}
\def\evq{{{\mymacro{ q}}}}
\def\evr{{{\mymacro{ r}}}}
\def\evs{{{\mymacro{ s}}}}
\def\evt{{{\mymacro{ t}}}}
\def\evu{{{\mymacro{ u}}}}
\def\evv{{{\mymacro{ v}}}}
\def\evw{{{\mymacro{ w}}}}
\def\evx{{{\mymacro{ x}}}}
\def\evy{{{\mymacro{ y}}}}
\def\evz{{{\mymacro{ z}}}}

\def\mA{{{\mymacro{ \mathbf{A}}}}}
\def\mB{{{\mymacro{ \mathbf{B}}}}}
\def\mC{{{\mymacro{ \mathbf{C}}}}}
\def\mD{{{\mymacro{ \mathbf{D}}}}}
\def\mE{{{\mymacro{ \mathbf{E}}}}}
\def\mF{{{\mymacro{ \mathbf{F}}}}}
\def\mG{{{\mymacro{ \mathbf{G}}}}}
\def\mH{{{\mymacro{ \mathbf{H}}}}}
\def\mI{{{\mymacro{ \mathbf{I}}}}}
\def\mJ{{{\mymacro{ \mathbf{J}}}}}
\def\mK{{{\mymacro{ \mathbf{K}}}}}
\def\mL{{{\mymacro{ \mathbf{L}}}}}
\def\mM{{{\mymacro{ \mathbf{M}}}}}
\def\mN{{{\mymacro{ \mathbf{N}}}}}
\def\mO{{{\mymacro{ \mathbf{O}}}}}
\def\mP{{{\mymacro{ \mathbf{P}}}}}
\def\mQ{{{\mymacro{ \mathbf{Q}}}}}
\def\mR{{{\mymacro{ \mathbf{R}}}}}
\def\mS{{{\mymacro{ \mathbf{S}}}}}
\def\mT{{{\mymacro{ \mathbf{T}}}}}
\def\mU{{{\mymacro{ \mathbf{U}}}}}
\def\mV{{{\mymacro{ \mathbf{V}}}}}
\def\mW{{{\mymacro{ \mathbf{W}}}}}
\def\mX{{{\mymacro{ \mathbf{X}}}}}
\def\mY{{{\mymacro{ \mathbf{Y}}}}}
\def\mZ{{{\mymacro{ \mathbf{Z}}}}}
\def\mBeta{{{\mymacro{ \boldsymbol{\beta}}}}}
\def\mPhi{{{\mymacro{ \boldsymbol{\Phi}}}}}
\def\mLambda{{{\mymacro{ \boldsymbol{\Lambda}}}}}
\def\mSigma{{{\mymacro{ \boldsymbol{\Sigma}}}}}



\def\gA{{{\mymacro{ \mathcal{A}}}}}
\def\gB{{{\mymacro{ \mathcal{B}}}}}
\def\gC{{{\mymacro{ \mathcal{C}}}}}
\def\gD{{{\mymacro{ \mathcal{D}}}}}
\def\gE{{{\mymacro{ \mathcal{E}}}}}
\def\gF{{{\mymacro{ \mathcal{F}}}}}
\def\gG{{{\mymacro{ \mathcal{G}}}}}
\def\gH{{{\mymacro{ \mathcal{H}}}}}
\def\gI{{{\mymacro{ \mathcal{I}}}}}
\def\gJ{{{\mymacro{ \mathcal{J}}}}}
\def\gK{{{\mymacro{ \mathcal{K}}}}}
\def\gL{{{\mymacro{ \mathcal{L}}}}}
\def\gM{{{\mymacro{ \mathcal{M}}}}}
\def\gN{{{\mymacro{ \mathcal{N}}}}}
\def\gO{{{\mymacro{ \mathcal{O}}}}}
\def\gP{{{\mymacro{ \mathcal{P}}}}}
\def\gQ{{{\mymacro{ \mathcal{Q}}}}}
\def\gR{{{\mymacro{ \mathcal{R}}}}}
\def\gS{{{\mymacro{ \mathcal{S}}}}}
\def\gT{{{\mymacro{ \mathcal{T}}}}}
\def\gU{{{\mymacro{ \mathcal{U}}}}}
\def\gV{{{\mymacro{ \mathcal{V}}}}}
\def\gW{{{\mymacro{ \mathcal{W}}}}}
\def\gX{{{\mymacro{ \mathcal{X}}}}}
\def\gY{{{\mymacro{ \mathcal{Y}}}}}
\def\gZ{{{\mymacro{ \mathcal{Z}}}}}

\def\sA{{{\mymacro{ \mathcal{A}}}}}
\def\sB{{{\mymacro{ \mathcal{B}}}}}
\def\sC{{{\mymacro{ \mathcal{C}}}}}
\def\sD{{{\mymacro{ \mathcal{D}}}}}
\def\sE{{{\mymacro{ \mathcal{E}}}}}
\def\sF{{{\mymacro{ \mathcal{F}}}}}
\def\sG{{{\mymacro{ \mathcal{G}}}}}
\def\sH{{{\mymacro{ \mathcal{H}}}}}
\def\sI{{{\mymacro{ \mathcal{I}}}}}
\def\sJ{{{\mymacro{ \mathcal{J}}}}}
\def\sK{{{\mymacro{ \mathcal{K}}}}}
\def\sL{{{\mymacro{ \mathcal{L}}}}}
\def\sM{{{\mymacro{ \mathcal{M}}}}}
\def\sN{{{\mymacro{ \mathcal{N}}}}}
\def\sO{{{\mymacro{ \mathcal{O}}}}}
\def\sP{{{\mymacro{ \mathcal{P}}}}}
\def\sQ{{{\mymacro{ \mathcal{Q}}}}}
\def\sR{{{\mymacro{ \mathcal{R}}}}}
\def\sS{{{\mymacro{ \mathcal{S}}}}}
\def\sT{{{\mymacro{ \mathcal{T}}}}}
\def\sU{{{\mymacro{ \mathcal{U}}}}}
\def\sV{{{\mymacro{ \mathcal{V}}}}}
\def\sW{{{\mymacro{ \mathcal{W}}}}}
\def\sX{{{\mymacro{ \mathcal{X}}}}}
\def\sY{{{\mymacro{ \mathcal{Y}}}}}
\def\sZ{{{\mymacro{ \mathcal{Z}}}}}

\def\emLambda{{\Lambda}}
\def\emA{{\mymacro{ A}}}
\def\emB{{\mymacro{ B}}}
\def\emC{{\mymacro{ C}}}
\def\emD{{\mymacro{ D}}}
\def\emE{{\mymacro{ E}}}
\def\emF{{\mymacro{ F}}}
\def\emG{{\mymacro{ G}}}
\def\emH{{\mymacro{ H}}}
\def\emI{{\mymacro{ I}}}
\def\emJ{{\mymacro{ J}}}
\def\emK{{\mymacro{ K}}}
\def\emL{{\mymacro{ L}}}
\def\emM{{\mymacro{ M}}}
\def\emN{{\mymacro{ N}}}
\def\emO{{\mymacro{ O}}}
\def\emP{{\mymacro{ P}}}
\def\emQ{{\mymacro{ Q}}}
\def\emR{{\mymacro{ R}}}
\def\emS{{\mymacro{ S}}}
\def\emT{{\mymacro{ T}}}
\def\emU{{\mymacro{ U}}}
\def\emV{{\mymacro{ V}}}
\def\emW{{\mymacro{ W}}}
\def\emX{{\mymacro{ X}}}
\def\emY{{\mymacro{ Y}}}
\def\emZ{{\mymacro{ Z}}}
\def\emSigma{{\mymacro{ \Sigma}}}

\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdata}{{\mymacro{ p_{\mathrm{data}}}}}
\newcommand{\ptrain}{{\mymacro{ \hat{p}_{\mathrm{data}}}}}
\newcommand{\Ptrain}{{\mymacro{ \hat{P}_{\mathrm{data}}}}}
\newcommand{\pmodel}{{\mymacro{ p_{\rm{model}}}}}
\newcommand{\Pmodel}{{\mymacro{ P_{\rm{model}}}}}
\newcommand{\ptildemodel}{{\mymacro{ \tilde{p}_{\rm{model}}}}}
\newcommand{\encoder}{{\mymacro{ \text{Enc}}}}
\newcommand{\decoder}{{\mymacro{ \text{Dec}}}}
\newcommand{\pencode}{{\mymacro{ p_{\rm{encoder}}}}}
\newcommand{\pdecode}{{\mymacro{ p_{\rm{decoder}}}}}
\newcommand{\precons}{{\mymacro{ p_{\rm{reconstruct}}}}}

\newcommand{\laplace}{\mathrm{Laplace}} %

\newcommand{\E}{{\mymacro{ \mathbb{E}}}}
\newcommand{\Ls}{{\mymacro{ \mathcal{L}}}}
\newcommand{\N}{{\mymacro{ \mathbb{N}}}}
\newcommand{\Nzero}{{\mymacro{ \mathbb{N}_{\geq 0}}}}
\newcommand{\emp}{{\mymacro{ \tilde{p}}}}
\newcommand{\lr}{{\mymacro{ \alpha}}}
\newcommand{\reg}{{\mymacro{ \lambda}}}
\newcommand{\rect}{{\mymacro{ \mathrm{rectifier}}}}
\newcommand{\projfunc}{{\mymacro{\boldsymbol{\pi}}}}
\newcommand{\projfuncEosalphabetminus}{{\mymacro{\vfunc}}}
\newcommand{\projfuncEosalphabetminusFunc}[1]{{\mymacro{\vfunc\left(#1\right)}}}
\newcommand{\tempParam}{{\mymacro{ \tau}}}
\newcommand{\KL}{{\mymacro{ D_{\mathrm{KL}}}}}
\newcommand{\Var}{{\mymacro{ \mathrm{Var}}}}
\newcommand{\standarderror}{{\mymacro{ \mathrm{SE}}}}
\newcommand{\Cov}{{\mymacro{ \mathrm{Cov}}}}


\newcommand{\loss}{{\mymacro{ \ell}}}
\newcommand{\softmax}{{\mymacro{ \mathrm{softmax}}}}
\newcommand{\sigmoid}{\mymacro{\mathrm{sigmoid}}}
\newcommand{\sparsemax}{{\mymacro{ \mathrm{sparsemax}}}}
\newcommand{\ReLU}{{\mymacro{ \mathrm{ReLU}}}}
\newcommand{\softmaxfunc}[2]{{\mymacro{ \mathrm{softmax}\!\left(#1\right)_{#2}}}} %
\newcommand{\sparsemaxfunc}[2]{{\mymacro{ \mathrm{sparsemax}\!\left(#1\right)_{#2}}}} %
\newcommand{\ReLUfunc}[1]{{\mymacro{ \ReLU\!\left(#1\right)}}} %
\newcommand{\determinant}[1]{{\mymacro{ \mathrm{det}\!\left(#1\right)}}}

\newcommand{\heaviside}{{\mymacro{ H}}}
\newcommand{\heavisideFun}[1]{{\mymacro{ \heaviside\left(#1\right)}}}
\newcommand{\sigmoidFun}[1]{{\mymacro{ \sigmoid\left(#1\right)}}}
\newcommand{\sigmoidVecPrime}[1]{{\mymacro{ \boldsymbol{\sigmoid}^\prime_{#1}}}}
\newcommand{\thrSigmoid}{{\mymacro{ \sigmoid_{\scaleto{\textnormal{T}}{4pt}}}}}
\newcommand{\softplus}{{\mymacro{ \zeta}}}
\newcommand{\clipping}{{\mymacro{ \mathrm{clip}}}}
\newcommand{\gradnorm}{{\mymacro{ \mathrm{gradnorm}}}}

\newcommand{\constbound}{{\mymacro{ M}}}
\newcommand*{\fpfull}{{\mymacro{ \texttt{float32}}}}
\newcommand{\normlzero}{{\mymacro{L^0}}}
\newcommand{\normlone}{{\mymacro{L^1}}}
\newcommand{\normltwo}{{\mymacro{L^2}}}
\newcommand{\normlp}{{\mymacro{L^p}}}
\newcommand{\normmax}{{\mymacro{L^\infty}}}

\newcommand{\matNormOne}[1]{{\mymacro{\norm{#1}_{1}}}}
\newcommand{\matNormTwo}[1]{{\mymacro{\norm{#1}_{2}}}}
\newcommand{\matNormP}[1]{{\mymacro{\norm{#1}_{p}}}}

\newcommand{\parents}{{\mymacro{Pa}}} %

\DeclareMathOperator*{\argmax}{{\mymacro{ argmax}}}
\DeclareMathOperator*{\argmin}{{\mymacro{ argmin}}}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}


\newcommand{\mop}[2]{[#1,#2]}
\newcommand{\mopt}[2]{[#1,#2]}
\newcommand{\mergetree}{{\mymacro{ \tau}}}
\newcommand{\mergetrees}{{\mymacro{ \ensuremath{\bm{\tau}}}}}
\newcommand{\amerge}{{\mymacro{ \mu}}}
\newcommand{\merges}{{\mymacro{ \boldsymbol{\merge}}}}
\newcommand{\validmerges}{{\mymacro{ \mathcal{M}_{\alphabetmerge} }}}
\newcommand{\encmerge}{{\mymacro{\textsf{apply}}}}
\newcommand{\singleencmerge}{{\mymacro{\textsf{singleapply}}}}
\newcommand{\yieldmerge}{{\mymacro{\textsf{yield}}}}
\newcommand{\treemerge}{{\mymacro{ \tau}}}
\newcommand{\treesmerge}{{\mymacro{ \ensuremath{\bm{\tau}}}}}
\newcommand{\bigO}[1]{{\mymacro{ \mathcal{O}\left(#1\right)}}}
\newcommand{\bigOmega}[1]{{\mymacro{ \Omega\left(#1\right)}}}
\newcommand{\mergesgreedy}{{\mymacro{ \merges^{\dagger}}}}
\newcommand{\mergesopt}{{\mymacro{ \merges^\star}}}
\newcommand{\computil}{{\mymacro{ \kappa}}}
\newcommand{\vnu}{{\mymacro{ \boldsymbol{\nu}}}}
\newcommand{\greedynu}{{\mymacro{ \nu^{\dagger}}}}
\newcommand{\optnu}{{\mymacro{ \nu^{\star}}}}
\newcommand{\prooftext}[1]{\text{\color{black!50}#1}}

\newcommand{\Jacobianhzero}{{\mymacro{ \frac{\partial \vhT}{\partial \vhzero}}}}
\newcommand{\Jacobianhtminus}{{\mymacro{ \frac{\partial \vht}{\partial \vhtminus}}}}
\newcommand{\activprimet}{{\mymacro{ \sigmoid'_{\tstep}}}}




\newcommand{\myQuad}{\hspace{0.7em}}
\newcommand*\circled[1]{\tikz[baseline=(char.base)]{%
            \node[shape=circle,draw,inner sep=1pt] (char) {\bfseries\small#1};}}


\newcommand{\hh}{\mymacro{\mathbf{h}}}
\newcommand{\bb}[1][]{\ifthenelse{\isempty{#1}}{\mymacro{\mathbf{b}}}{\mymacro{\mathbf{b}^{\text{#1}}}}}
\newcommand{\ff}[1][]{\ifthenelse{\isempty{#1}}{\mymacro{f}}{\mymacro{f_{\text{#1}}}}}
\newcommand{\qq}{\mymacro{\mathbf{q}}}
\newcommand{\kk}{\mymacro{\mathbf{k}}}

\newcommand{\FF}{\mymacro{\mathbf{F}}}
\newcommand{\GG}{\mymacro{\mathbf{G}}}
\newcommand{\X}{\mymacro{\mathbf{X}}}
\newcommand{\Y}{\mymacro{\mathbf{Y}}}
\newcommand{\M}{\mymacro{\mathbf{M}}}
\newcommand{\SSS}{\mymacro{\mathbf{S}}}
\newcommand{\W}[1][]{\ifthenelse{\isempty{#1}}{\mymacro{\boldsymbol{\Theta}}}{\mymacro{\boldsymbol{\Theta}^{\text{#1}}}}}
\newcommand{\A}{\mymacro{\mathbf{A}}}
\newcommand{\calA}{\mymacro{\mathcal{A}}}
\newcommand{\aaa}{\mymacro{\mathbf{a}}}
\newcommand{\mm}{\mymacro{\mathbf{m}}}
\newcommand{\ww}{\mymacro{\boldsymbol{w}}}
\newcommand{\hw}{\mymacro{\widehat{w}}}
\newcommand{\aalpha}{\mymacro{\boldsymbol{\alpha}}}
\newcommand{\e}{\mymacro{e}}


\newcommand{\stacktop}[1][]{\ifthenelse{\isempty{#1}}{\mymacro{\gamma^{\text{top}}}}{\mymacro{\gamma^{\text{top}}_{#1}}}}
\newcommand{\sym}{\strcolor{\texttt{w}}}
\newcommand{\syma}{\strcolor{\texttt{a}}}
\newcommand{\symb}{\strcolor{\texttt{b}}}
\newcommand{\symc}{\strcolor{\texttt{c}}}
\newcommand{\symd}{\strcolor{\texttt{d}}}
\newcommand{\symu}{\strcolor{\texttt{u}}}
\newcommand{\symM}{\strcolor{\texttt{M}}}
\newcommand{\symP}{\strcolor{\texttt{P}}}

\newcommand{\bool}{\mymacro{\mathbb{B}}}

\newcommand{\lang}{{\strcolor{ L}}}
\newcommand{\langfun}{{\strcolor{\mathbb{L}}}}

\newcommand{\push}{\mymacro{\texttt{PUSH}}}
\newcommand{\pop}{\mymacro{\texttt{POP}}}
\newcommand{\noop}{\mymacro{\texttt{NO-OP}}}
\newcommand{\peek}{\mymacro{\texttt{PEEK}}}
\newcommand{\onehot}[1][]{\ifthenelse{\isempty{#1}}{\mymacro{ \llbracket \rrbracket}}{\mymacro{ \llbracket#1\rrbracket}}}

\newcommand{\tquery}{\mymacro{\text{(query)}}}
\newcommand{\tkey}{\mymacro{\text{(key)}}}
\newcommand{\tvalue}{\mymacro{\text{(value)}}}

\newcommand{\nope}{\mymacro{\texttt{NoPE}}}
\newcommand{\sincos}{\mymacro{\texttt{SiPE}}}
\newcommand{\relative}{\mymacro{\texttt{relative}}}
\newcommand{\rotary}{\mymacro{\texttt{RoPE}}}
\newcommand{\ALiBi}{\mymacro{\texttt{ALiBi}}}

\newcommand{\FFN}{\mymacro{\text{FFN}}}
\newcommand{\MHA}{\mymacro{\mathbf{M}}}
\newcommand{\LN}{\mymacro{\text{LN}}}
\newcommand{\Stack}{\mymacro{\mathbf{S}}}
\newcommand{\embedding}{\mymacro{\mathbf{E}}}
\newcommand{\classification}{\mymacro{c}}
\newcommand{\cls}{\mymacro{o}}

\newcommand{\stackop}{\mymacro{\upsilon}}

\newcommand{\domain}[1]{\mymacro{\text{dom}(#1)}}
\newcommand{\image}[1]{\mymacro{\text{im}(#1)}}

\newcommand{\opsince}{\mymacro{\mathrel{\textbf{S}}}}
\newcommand{\opuntil}{\mymacro{\mathrel{\textbf{U}}}}

\newcommand{\sfclass}{\mymacro{\mathcal{V}}}
\newcommand{\foclass}{\mymacro{\Sigma}}
\newcommand{\raspclass}{\mymacro{\mathcal{B}}}


\newcommand{\qd}{\mymacro{\text{qd}}}
\newcommand{\od}{\mymacro{\text{od}}}


\makeatletter
\newcommand*{\bigcdot}{}%
\DeclareRobustCommand*{\bigcdot}{%
  \mathbin{\mathpalette\bigcdot@{}}%
}
\newcommand*{\bigcdot@scalefactor}{.5}
\newcommand*{\bigcdot@widthfactor}{1.15}
\newcommand*{\bigcdot@}[2]{%
  \sbox0{$#1\vcenter{}$}%
  \sbox2{$#1\cdot\m@th$}%
  \hbox to \bigcdot@widthfactor\wd2{%
    \hfil
    \raise\ht0\hbox{%
      \scalebox{\bigcdot@scalefactor}{%
        \lower\ht0\hbox{$#1\bullet\m@th$}%
      }%
    }%
    \hfil
  }%
}
\makeatother



\newcommand{\true}{\mymacro{\top}}
\newcommand{\TRUE}{\mymacro{\textsc{true}}}
\newcommand{\false}{\mymacro{\bot}}
\newcommand{\FALSE}{\mymacro{\textsc{false}}}

\newcommand{\past}{\opcolor{\mathrel{\textup{\textbf{P}}}}}
\newcommand{\future}{\opcolor{\mathrel{\textup{\textbf{F}}}}}
\newcommand{\pasteq}{\opcolor{\past}^{=}}
\newcommand{\prev}[1][]{\ifthenelse{\isempty{#1}}{\opcolor{\mathrel{\textup{\textbf{Y}}}}}{\opcolor{\mathrel{\textup{\textbf{Y}}}}^{\leq #1}}}
\newcommand{\prevstar}{\opcolor{\mathrel{\textup{\textbf{Y}}}}^{*}}
\newcommand{\nxt}{\opcolor{\mathrel{\textup{\textbf{X}}}}}
\newcommand{\since}{\opcolor{\mathrel{\textup{\textbf{S}}}}}
\newcommand{\until}{\opcolor{\mathrel{\textup{\textbf{U}}}}}

\newcommand{\ltl}{\ltlcolor{\textup{\textbf{LTL}}}[\since]}
\newcommand{\tl}{\ltlcolor{\textup{\textbf{LTL}}}[\past,\future]}
\newcommand{\ptl}{\ltlcolor{\textup{\textbf{LTL}}}\left[\past\right]}
\newcommand{\yptl}[1][]{\ltlcolor{\textup{\textbf{LTL}}}\left[\past,\prev[#1]\right]}
\newcommand{\ytl}[1][]{\ltlcolor{\textup{\textbf{LTL}}}\left[\prev[#1]\right]}
\newcommand{\rtl}{\ltlcolor{\textup{\textbf{LTL}}}\left[\pasteq,\prev\right]}
\newcommand{\gtl}[1]{\ltlcolor{\textup{\textbf{LTL}}}[#1]}

\newcommand{\dimension}[1][]{\ifthenelse{\isempty{#1}}{\mymacro{D}}{\mymacro{D}_{\text{#1}}}}
\newcommand{\length}{N}
\newcommand{\layernumber}{\mymacro{L}}
\newcommand{\headnumber}{\mymacro{H}}
\newcommand{\localnumber}{\mymacro{H_{\prev}}}
\NewDocumentCommand{\transformer}{O{} O{} O{} o }{
  \IfBlankTF{#1}{
    \IfBlankTF{#2}{
      \IfNoValueTF{#4}{\rmH}{\rmH(#4)}
    }{
      \IfNoValueTF{#4}{\mymacro{\rmH_{#2,#3}}}{\mymacro{\rmH(#4)_{#2,#3}}}
    }
  }{
    \IfBlankTF{#2}{
      \IfNoValueTF{#4}{\mymacro{\rmH^{#1}}}{\mymacro{\rmH^{#1}(#4)}}
    }{
      \IfNoValueTF{#4}{\mymacro{\rmH^{#1}_{#2,#3}}}{\mymacro{\rmH^{#1}(#4)_{#2,#3}}}
    }
  }
}

\NewDocumentCommand{\halftransformer}{O{} O{} O{} o }{
  \IfBlankTF{#1}{
    \IfBlankTF{#2}{
      \IfNoValueTF{#4}{\rmG}{\rmG(#4)}
    }{
      \IfNoValueTF{#4}{\mymacro{\rmG_{#2,#3}}}{\mymacro{\rmG(#4)_{#2,#3}}}
    }
  }{
    \IfBlankTF{#2}{
      \IfNoValueTF{#4}{\mymacro{\rmG^{#1}}}{\mymacro{\rmG^{#1}(#4)}}
    }{
      \IfNoValueTF{#4}{\mymacro{\rmG^{#1}_{#2,#3}}}{\mymacro{\rmG^{#1}(#4)_{#2,#3}}}
    }
  }
}
\NewDocumentCommand{\attention}{o}{\IfNoValueTF{#1}{\mymacro{\mathbf{A}}}{\mymacro{\mathbf{A}^{#1}}}}
\NewDocumentCommand{\ffn}{o}{\IfNoValueTF{#1}{\mymacro{\mathbf{F}}}{\mymacro{\mathbf{F}^{#1}}}}
\NewDocumentCommand{\fo}{o}{\IfNoValueTF{#1}{\mymacro{\textbf{FO}[\mathord<]}}{\mymacro{\textbf{FO}^{#1}[\mathord<]}}}
\NewDocumentCommand{\pfo}{o}{\IfNoValueTF{#1}{\mymacro{\textbf{PFO}^2[\mathord<]}}{\mymacro{\textbf{PFO}^2[\mathord<,#1]}}}

\newcommand{\fof}{\fmcolor{\phi}}
\newcommand{\tlf}{\fmcolor{\psi}}
\newcommand{\atom}{\fmcolor{\pi}}

\newcommand{\fpnset}{\mymacro{\mathbb{F}}}
\newcommand{\nnfpnset}{\mymacro{\mathbb{F}_{\geq 0}}}
\newcommand{\fpn}{\mymacro{f}}

\NewDocumentCommand{\query}{o o }{\IfNoValueTF{#1}{\rmQ}{\rmQ_{#1,#2}}}
\NewDocumentCommand{\key}{o o }{\IfNoValueTF{#1}{\rmK}{\rmK_{#1,#2}}}
\NewDocumentCommand{\val}{o o }{\IfNoValueTF{#1}{\rmV}{\rmV_{#1,#2}}}
\newcommand{\score}{\mymacro{\mathbf{S}}}
\newcommand{\mask}{\mymacro{\mathbf{M}}}
\NewDocumentCommand{\localmask}{o o }{\IfNoValueTF{#1}{\rmM^{\leq k}}{\rmM^{\leq k}_{#1,#2}}}
\NewDocumentCommand{\globalmask}{o o }{\IfNoValueTF{#1}{\rmM^{*}}{\rmM^{*}_{#1,#2}}}

\newcommand{\morphism}{\mymacro{\mu}}

\newcommand{\equivalent}{\mymacro{\equiv_\lang}}

\newcommand{\ltod}{\mymacro{g}}
\newcommand{\stod}{\mymacro{h}}

\newcommand{\maxfpn}{\mymacro{\textsc{max}}}
\newcommand{\minfpn}{\mymacro{\textsc{min}}}

\newcommand{\nmax}{\mymacro{n_{\max}}}

\newcommand{\monoid}{\algmacro{\mathbb{M}}}
\newcommand{\submonoid}{\mymacro{\mathbb{N}}}
\newcommand{\semigroup}{\algmacro{\mathbb{S}}}
\newcommand{\idem}{\mymacro{e}}

\NewDocumentCommand{\ball}{m}{\mymacro{\B_{#1}}}

\newcommand{\pe}{\mymacro{\theta}}

\newcommand{\plm}{\mymacro{p}}
\newcommand{\localplm}{\mymacro{\overrightarrow{p}}}
\newcommand{\blm}{\mymacro{q}}
\newcommand{\localblm}{\mymacro{\overrightarrow{q}}}

\newcommand{\reject}{\mymacro{\stateq_{-1}}}
\newcommand{\gtrans}{\mymacro{\Delta}}
\newcommand{\outgoing}{\mymacro{\mathcal{E}}}
\newcommand{\unkoutgoing}{\mymacro{\underline{\outgoing}}}

\newcommand{\unkalphabet}{\mymacro{\underline{\overline{\alphabet}}}}
\newcommand{\unkltod}{\mymacro{\underline{\ltod}}}
\newcommand{\rejstates}{\mymacro{\underline{\states}}}

\newcommand{\factor}{\mymacro{\mathbb{I}}}
\newcommand{\suffix}{\mymacro{S}}
\newcommand{\suffixset}{\mymacro{\mathbb{S}}}
\newcommand{\prefix}{\mymacro{P}}
\newcommand{\prefixset}{\mymacro{\mathbb{P}}}
\newcommand{\ssym}{\mymacro{\rtimes}}
\newcommand{\esym}{\mymacro{\ltimes}}

\RenewDocumentCommand{\mod}{ o o }{%
  \mymacro{\mathrm{MOD}%
  \IfValueT{#1}{_{#1}}%
  \IfValueT{#2}{^{#2}}%
  }
}

